Langevin Monte Carlo for strongly log-concave distributions: Randomized midpoint revisited

We revisit the problem of sampling from a target distribution that has a smooth strongly log-concave density everywhere in $\mathbb R^p$. In this context, if no additional density information is available, the randomized midpoint discretization for the kinetic Langevin diffusion is known to be the most scalable method in high dimensions with large condition numbers. Our main result is a nonasymptotic and easy to compute upper bound on the Wasserstein-2 error of this method. To provide a more thorough explanation of our method for establishing the computable upper bound, we conduct an analysis of the midpoint discretization for the vanilla Langevin process. This analysis helps to clarify the underlying principles and provides valuable insights that we use to establish an improved upper bound for the kinetic Langevin process with the midpoint discretization. Furthermore, by applying these techniques we establish new guarantees for the kinetic Langevin process with Euler discretization, which have a better dependence on the condition number than existing upper bounds.

==> Sections/notation.tex <==
\usepackage[utf8]{inputenc}
\usepackage[dvipsinames]{xcolor}
% \definecolor{bordeau}{rgb}{0.3515625,0,0.234375}
\usepackage[absolute,overlay]{textpos}
\usepackage{graphicx} 

\usepackage{lipsum}
\usepackage{array}
\usepackage{caption}
% \usepackage{capt-of}
\usepackage{multicol}
\usepackage{hyperref}
\usepackage{afterpage}
\usepackage{setspace}
\usepackage{diagbox}
\usepackage{pgffor}

\usepackage{comment}

\setlength{\columnseprule}{0pt}
\setlength\columnsep{10pt}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage
}

%Bibliography style
\usepackage{natbib}[square, numbers]
\bibliographystyle{alpha}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{dsfont}            % for indicator function
% \usepackage{bbold}
\usepackage{import}
\usepackage[toc,page]{appendix}
\usepackage{minitoc}

% Make the "Part I" text invisible
% \renewcommand \thepart{}
% \renewcommand \partname{}
% \usepackage{tocloft}
% \renewcommand{\cftsecleader}{\cftdotfill{\cftdotsep}}

%\documentclass[a4paper,sts,preprint,reqno,usenames,dvipsnames]{imsart}
%\usepackage[utf8]{inputenc}
\usepackage{amsmath}
%\usepackage[left=3cm,right=3cm,top=3cm,bottom=3cm]{geometry}
%\usepackage{mathtools}
\usepackage{amssymb,amsthm}
\usepackage{graphicx}
% \usepackage[dvipsnames]{xcolor}

\usepackage{mathrsfs}
\usepackage{nicefrac}

\definecolor{darkmidnightblue}{HTML}{003366}    
\definecolor{midnightblue}{HTML}{0059b3}
\definecolor{chromered}{HTML}{f14233}


\definecolor{darkpowderblue}{rgb}{0.0, 0.2, 0.6}
\definecolor{dukeblue}{rgb}{0.0, 0.0, 0.61}

%\RequirePackage
%[colorlinks,citecolor=blue,urlcolor=blue,breaklinks=true]
        %{hyperref}
\hypersetup{
    colorlinks = true,
    citecolor= darkmidnightblue,
    urlcolor=darkmidnightblue,
    breaklinks=true,
    linkcolor = darkmidnightblue,
    linkbordercolor = {white},
}
% \usepackage{natbib}%[round,sort]
% \bibliographystyle{apa}

\usepackage{cleveref}
\usepackage{autonum}
\usepackage{algorithm}
\usepackage{algorithmic}

\newcommand{\sqN}[1]{\Norm{#1}^2}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\normsq}[1]{\left\| #1 \right\|^2}
\newcommand{\inner}[2]{\left< #1 , #2 \right>}

\newcommand{\brr}[1]{\left( #1 \right)}   % brackets round
\newcommand{\brs}[1]{\left[ #1 \right]}  % brackets square
\newcommand{\brc}[1]{\left\{ #1 \right\}} % brackets curly

%%%% LAST PAGE
\usepackage[absolute,overlay]{textpos}



\parskip=5pt

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
    \def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand\prob{\mathbb{P}}
\newcommand\indic{\mathds{1}}
\newcommand\dx{\mathrm{d}x}
\newcommand\dy{\mathrm{d}y}
\newcommand\cvn{\underset{n\rightarrow\infty}{\rightarrow}}
\newcommand\cvps{\overset{p.s.}{\rightarrow}}
\newcommand\cvprob{\overset{\prob}{\rightarrow}}
\newcommand\cvloi{\overset{\mathcal{L}}{\rightarrow}}
\newcommand\Xbar{\overline{X}_n}
\newcommand\calX{\mathcal{X}}
\newcommand\calP{\mathcal{P}}
\newcommand\calN{\mathcal{N}}
\newcommand\calL{\mathcal{L}}

\newcommand\bs{\boldsymbol}

\newcommand\bB{\boldsymbol B}
\newcommand\bD{\boldsymbol D}
\newcommand\bfD{\mathbf D}
\newcommand\bfC{\mathbf C}
\newcommand\bfE{\mathbf E}
\newcommand\bfP{\mathbf P}
\newcommand\bfQ{\mathbf Q}
\newcommand\bfN{\mathbf N}
\newcommand\bfSigma{\mathbf\Sigma}
\newcommand\bfH{\mathbf H}
\newcommand\bfR{\mathbf R}
\newcommand\R{\mathbb R}
\newcommand\bfS{\mathbf S}
\newcommand\bfM{\mathbf M}
\newcommand\bL{\boldsymbol L}
\newcommand\bY{\boldsymbol Y}
\newcommand\bP{\boldsymbol P}
\newcommand\bQ{\boldsymbol Q}
\newcommand\bR{\boldsymbol R}
\newcommand\bA{\boldsymbol A}
\newcommand\bC{\boldsymbol C}
\newcommand\bX{\boldsymbol X}
\newcommand\bZ{\boldsymbol Z}
\newcommand\bW{\boldsymbol W}


\newcommand\bh{\boldsymbol h}
\newcommand\bx{\boldsymbol x}
\newcommand\by{\boldsymbol y}
\newcommand\bz{\boldsymbol z}

\newcommand\bu{\boldsymbol u}
\newcommand\bv{\boldsymbol v}
\newcommand\bw{\boldsymbol w}
\newcommand\bl{\boldsymbol l}
\newcommand\bU{\boldsymbol U}
\newcommand\bV{\boldsymbol V}
\newcommand\bg{\boldsymbol g}
\newcommand\bxi{\boldsymbol\xi}
\newcommand\bmu{\boldsymbol\mu}
\newcommand\NN{\mathbb N}
\newcommand\RR{\mathbb R}
\newcommand\EE{\mathbb E}
\newcommand\E{\mathbb E}
\newcommand\CC{\mathbb C}
\newcommand\LL{\mathbb L}
\newcommand\Ltwo{\mathbb L_2}
\newcommand\Cov{\textbf{Cov}}
\newcommand\Var{\textbf{Var}}
\newcommand\Exp{\textbf E}
\newcommand\bfI{\mathbf I}
% \newcommand\bfO{\mathbf O}
\newcommand\bfA{\mathbf A}
\newcommand\bfB{\mathbf B}
\newcommand{\bS}{\boldsymbol S}
\newcommand{\eeta}{\boldsymbol{\eta}}
\newcommand{\bfeta}{{\boldsymbol{\eta}}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\DeclareMathOperator{\tr}{tr}

\newcommand\eps{\varepsilon}
\newcommand\bzeta{\bs \zeta}
\newcommand\bta{ \bs \eta}
\newcommand\tdkappa{\tilde{\kappa}}
\newcommand\bDelta{\boldsymbol\Delta}

\newcommand\btheta{\boldsymbol\theta}
\newcommand\bvartheta{\boldsymbol\vartheta}
\def\Tilde{\widetilde}
\def\tilde{\widetilde}
\def\hat{\widehat}
\def\ds{\displaystyle}
\def\bfE{\mathbf E}
\def\DKL{D_{\rm KL}}
\def\dTV{d_{\rm TV}}
\def\dbL{d_{\rm bL}}



\newcommand{\SCGL}[2]{\hyperlink{SCGL}
{{\textupsf{{$({#1},{#2})$-SCGL}}}}}


\newcommand{\textupsf}[1]{\textup{\textsf{#1}}}
\def\CLPEN1{\hyperlink{PEN}{\textupsf{{$(C,\lambda)$-PEN}}}}

\def\PLD1{\hyperlink{PLD}{\textupsf{{PLD}}}}
\def\PGF1{\hyperlink{PGF}{\textupsf{{PGF}}}}
\def\TPLD1{\hyperlink{TPLD}{\textupsf{{TPLD}}}}
\newcommand{\AssA}[2]{\hyperlink{AssA}{\textup{\textbf{A}}}$({#1},{#2})$}

\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{condition}{Condition}
\newtheorem{lemma}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{corollary}{Corollary}
\newtheorem{defin}{Definition}
\newtheorem{remark}{Remark}


\crefname{cor}{Corollary}{Corollaries}
\crefname{condition}{Condition}{C}


\renewcommand{\familydefault}{\rmdefault}


\newcommand{\grad}{\nabla}

\newcommand{\normtwo}[1]{ \ensuremath{\left\| #1 \right\|_{2} }}

\newcommand{\argmin}{\mathop{\mathrm{arg\,min}}}


\newcommand{\id}{\ensuremath{\mathbf{I}}}



\newcommand{\ly}[1]{{\color{magenta}LY: #1}}


\newcommand{\bigo}{\mathcal{O}}



==> Sections/rklmc.tex <==
% !TEX root = ../main.tex


\newpage
\section{Improved bounds on the error of KLMC 
in Wasserstein-2 distance}


We consider the discretization version of KLMC
    \begin{align}
        \bv_{n+1} & = \bv_n e^{-\gamma h}  - \int_0^h e^{-\gamma(h-s)}\,ds 
        \nabla f(\btheta_n) + \sqrt{2\gamma} \int_0^h e^{-\gamma(h-s)}\,d\bW_s\\
        \btheta_{n+1} & = \btheta_n + \int_0^h \bigg(\bv_n e^{-\gamma u}  - \int_0^u e^{-\gamma(u-s)}\,ds 
        \nabla f(\btheta_n) + \sqrt{2\gamma} \int_0^u e^{-\gamma(u-s)}\,d\bW_s
        \bigg)\,du\,.
    \end{align}
To derive the convergence rate of KLMC, we introduce the following integral formulation, which is the solution to the SDE~\eqref{eq:uld} at time $t$ with initial value $(\btheta_n,\bv_n)$
\begin{align}
\bv_{n}^*(t) & = \bv_n e^{-\gamma t}  - \int_0^t e^{-\gamma(t-s)}
        \nabla f(\btheta^*_n(s))\,ds + \sqrt{2\gamma} \int_0^t e^{-\gamma(t-s)}\,d\bW_s\\
\btheta_{n}^*(t) & = \btheta_n + \int_0^t \bv^*_n(s)\,ds\,.
\end{align}
Given the step size $h>0,$ we set the 1-step exact Langevin diffusion starting from $(\btheta_n,\bv_n)$ as
\begin{align}
\bv_{n+1}^*=\bv_{n}^*(h),\quad 
\btheta_{n+1}^*=\btheta_{n}^*(h)\,.
\end{align}

\begin{lemma}
\label{lem:klmc}
If for some $M\geqslant 0$, the gradient $\nabla f$ 
is $M$-Lipschitz continuous, then for every step-size 
$h\geqslant 0$ and every $\gamma\geqslant 0$, it holds that
\begin{align}
\norm{\bv_{k+1}-\bv_{k+1}^*}_{\Ltwo}
& \leqslant  0.5 Mh^2e^{Mh^2/2} (0.8\sqrt{\gamma dh }
+\norm{\bv_k}_{\Ltwo}
+0.4 h\norm{\grad f(\btheta_k)}_{\Ltwo}) \\
\norm{\btheta_{k+1}-\btheta_{k+1}^*}_{\Ltwo}
& \leqslant  (1/6)Mh^3e^{Mh^2/2} (0.7\sqrt{\gamma dh }
+\norm{\bv_k}_{\Ltwo}
+0.25 h\norm{\grad f(\btheta_k)}_{\Ltwo}) \,.
\label{eq:thetadiff}
\end{align}
\end{lemma}
\begin{proof}
[Proof of Lemma~\ref{lem:klmc}]

{\color{blue}
Notice that
\begin{align}
    \|e^{\gamma t} \bv_n^*(t) -\bv_n^*(0)\|_{\mathbb L_2}^2 &=\bigg\|\int_0^t e^{\gamma s}\nabla f(\btheta^*(s))\,ds\bigg\|_{\mathbb L_2}^2 + 2\gamma p\int_0^t
    e^{2\gamma s}\,ds\\
    &\leqslant \bigg\{
     M \int_0^t e^{\gamma s}\big\|\btheta^*(s)-\btheta_n\big\|_{\mathbb L_2}\,ds + 
    \int_0^t e^{\gamma s}\,ds\|\nabla f(\btheta^*(s))\|_{\mathbb L_2}\bigg\}^2 + 2\gamma p\int_0^t
    e^{2\gamma s}\,ds\\
    &\leqslant \bigg\{
     M \int_0^t e^{\gamma s}\int_0^s\big\|\bv^*_n(u)\big\|_{\mathbb L_2}\,du\,ds + 
    \int_0^t e^{\gamma s}\,ds\|\nabla f(\btheta^*(s))\|_{\mathbb L_2}\bigg\}^2 + 2\gamma p\int_0^t
    e^{2\gamma s}\,ds\\
    &= \bigg\{
     M \int_0^t \int_0^{t-u}e^{\gamma z}\,dz \big\|e^{\gamma u}\bv^*_n(u)\big\|_{\mathbb L_2}\,du + 
    \int_0^t e^{\gamma s}\,ds\|\nabla f(\btheta^*(s))\|_{\mathbb L_2}\bigg\}^2 + 2\gamma p\int_0^t
    e^{2\gamma s}\,ds
\end{align}

}
We note that
 \begin{align}
e^{\gamma h}\big(\bv_{n}(h) - \bv_{n}^*(h)\big) 
 &= \int_0^h e^{\gamma s}\big(\nabla f(\btheta_n^*(s)) - \nabla f(\btheta_n)\big)\,ds\\
 &= \int_0^h e^{\gamma s}\underbrace{\Big\{\int_0^1\nabla f^2(z\btheta_n^*(s) + (1-z)\btheta_n)\,dz\Big\}}_{:=\bfH(s)} \big(\btheta_n^*(s) - \btheta_n\big)\,ds\\
& = \int_0^h e^{\gamma s} \bfH(s) \int_0^s \bv_n^*(u)\,du\,ds.\\
& = \int_0^h \int_u^h e^{\gamma s} \bfH(s) \,ds  \bv_n^*(u)\,du\\
& = \int_0^h \int_0^{h-u} e^{\gamma z} \bfH(u + z) \,dz  \,e^{\gamma u}\bv_n^*(u)\,du
\label{lem21:1}
\end{align}
On the one hand, for every $s\in[0,h]$, we have
\begin{align}
\btheta^*_n(t) - \btheta_n 
&= \int_0^t \bv^*_n(s) ds\\
&= -\int_0^t \int_0^s e^{\gamma (u-s)}\nabla f(\btheta^*_n(u))\,du\,ds 
+ \bv_n \int_0^t e^{-\gamma s}\,ds\\
&= -\int_0^t \nabla f(\btheta^*_n(u))\,\int_0^{t-u} 
e^{-\gamma z}dz\,du 
+ \bv_n \int_0^t e^{-\gamma s}\,ds\\
        \label{lem21:2}
    \end{align}
 On the other hand, for every $u\in[0,h]$, we have
\begin{align}
\big\|\bv^*_n(u) - \bv_{n}e^{-\gamma u}\big\|_{\mathbb L_2}
&\leqslant  
\bigg\|\int_0^u e^{-\gamma(u-t)} \big(\nabla f(\btheta^*_n(t))-\nabla f(\btheta_n)\big)\,dt\bigg\|_{\mathbb L_2} 
+ \bigg\|\int_0^u e^{-\gamma(u-t)} \nabla f(\btheta_n)\,dt\bigg\|_{\mathbb L_2} \\ 
&\qquad + \sqrt{2\gamma} \bigg\|\int_0^u e^{-\gamma(u-t)}\,d\bW_t\bigg\|_{\mathbb L_2}\\
&\leqslant  \int_0^u \big\|\nabla f(\btheta^*_n(t))-\nabla f(\btheta_n) \big\|_{\mathbb L_2}\,dt 
+\int_0^u \big\| \nabla f(\btheta_n)\big\|_{\mathbb L_2}\,dt
+ \sqrt{2\gamma d u}\\
&\leqslant  M\int_0^u \big\|\btheta^*_n(t)-\btheta_n \big\|_{\mathbb L_2}\,dt 
+ u\big\| \nabla f(\btheta_n)\big\|_{\mathbb L_2}
+ \sqrt{2\gamma du}. 
\label{lem21:3}
\end{align}
Combining \eqref{lem21:2} and \eqref{lem21:3}, we arrive at
\begin{align}
\big\|\btheta^*_n(t) - \btheta_n\big\|_{\mathbb L_2} 
&\leqslant 
\int_0^s \big(M\int_0^u \big\|\btheta^*_n(t)-\btheta_n \big\|_{\mathbb L_2}\,dt 
+u\big\| \nabla f(\btheta_n)\big\|_{\mathbb L_2}
+ \sqrt{2\gamma du}\big)\,du
+ s\|\bv_n\|_{\mathbb L_2} \\
&\leqslant  
M \int_0^s (s-t) \big\|\btheta^*_n(t)-\btheta_n \big\|_{\mathbb L_2}\,dt   +\sqrt{(8/9)\gamma ds^3} 
+ s\|\bv_n\|_{\mathbb L_2}
+ 0.5s^2\|\grad f(\btheta_n)\|_{\mathbb L_2} \\
&\leqslant  M \int_0^s (h-t) \big\|\btheta^*_n(t)-\btheta_n \big\|_{\mathbb L_2}\,dt   +\sqrt{(8/9)\gamma ds^3} 
+ s\|\bv_n\|_{\mathbb L_2}
+ 0.5s^2\|\grad f(\btheta_n)\|_{\mathbb L_2} .
\label{lem21:4}
\end{align}
The last inequality allows us to use the Gronwall lemma, which implies that
\begin{align}
\big\|\btheta^*_n(t) - \btheta_n\big\|_{\mathbb L_2} 
&\leqslant  \big(\sqrt{(8/9)\gamma ds^3} + s\|\bv_n\|_{\mathbb L_2}
+0.5s^2\|\grad f(\btheta_n)\|_{\mathbb L_2}
\big)
 e^{Ms(h-s/2)}\\
 &\leqslant \big(\sqrt{(8/9)\gamma ds^3} + s\|\bv_n\|_{\mathbb L_2}
 + 0.5s^2\|\grad f(\btheta_n)\|_{\mathbb L_2}\big)e^{Mh^2/2}.
\label{lem21:5}
\end{align}
Combining the last display with \eqref{lem21:1}, we get
\begin{align}
\big\|\bv_{n+1} - \bv_{n+1}^*\big\|_{\mathbb L_2} 
&\leqslant  M e^{Mh^2/2} \int_0^h \big(\sqrt{(8/9)\gamma ds^3} 
+ s\|\bv_n\|_{\mathbb L_2}
+0.5s^2\|\grad f(\btheta_n)\|_{\mathbb L_2}\big)\,ds\\
&\leqslant  \frac{4\sqrt{2\gamma d} Me^{Mh^2/2}}{15}\,h^{5/2} 
+ 0.5 Mh^2 e^{Mh^2/2}\|\bv_n\|_{\mathbb L_2}
+ \frac{1}{6}Mh^3 e^{Mh^2/2} \norm{\grad f(\btheta_n)}_{\Ltwo}\\
&\leqslant 0.5 Mh^2 e^{Mh^2/2} (0.8\sqrt{\gamma dh} + 
\|\bv_n\|_{\mathbb L_2}+ 0.4h\norm{\grad f(\btheta_n)}_{\Ltwo}).
\label{lem21:6}
\end{align}
This completes the proof of the first inequality. To prove the second 
one, one can note that
\begin{align}
\big\|\btheta_{n+1} - \btheta_{n+1}^*\big\|_{\mathbb L_2} 
&= \bigg\|\int_0^h \int_0^t e^{-\gamma(t-s)}\big(\nabla f(\btheta_n^*(s)) - \nabla f(\btheta_n)\big)\,ds \,dt \bigg\|_{\mathbb L_2}\\
 &\leqslant  \int_0^h\int_0^t \big\|\nabla f (\btheta_n^*(s)) 
- \nabla f(\btheta_n)\big\|_{\mathbb L_2}\,ds \,dt \\
&\leqslant  M \int_0^h\int_0^t \big\|\btheta_n^*(s) 
- \btheta_n\big\|_{\mathbb L_2}\,ds \,dt.
\end{align}
The last term can be bounded using \eqref{lem21:5}. 
This yields
\begin{align}
\big\|\btheta_{n+1} - \btheta_{n+1}^*\big\|_{\mathbb L_2} 
& \leqslant  M e^{Mh^2/2} \int_0^h\int_0^t 
\big(\sqrt{(8/9)\gamma ds^3} 
+ s\|\bv_n\|_{\mathbb L_2}
+0.5s^2\|\grad f(\btheta_n)\|_{\mathbb L_2}
\big)\,ds \,dt\\
& \leqslant  {\frac{4Mh^3 }{35} e^{Mh^2/2} 
\sqrt{(8/9)\gamma d h} 
+ \frac{M}{6} e^{Mh^2/2}\|\bv_n\|_{\mathbb L_2}h^3}
+ \frac{Mh^4}{24}e^{Mh^2/2}  \norm{\grad f(\btheta_n)}_{\Ltwo}\\
&\leqslant (1/6) Mh^3 e^{Mh^2/2} \big(0.7\sqrt{\gamma dh} 
+ \|\bv_n\|_{\mathbb L_2}
+ 0.25h \norm{\grad f(\btheta_n)}_{\Ltwo}\big)
\end{align}
as desired.
\end{proof}

In what follows, we rewrite the iterates of the KLMC in the form
\begin{align}
    \bv_{n+1} & = (1- \alpha \gamma h) \bv_n  - \alpha h 
        \nabla f(\btheta_n) + \sqrt{2\gamma h} \sigma \bxi_n \label{vn1}\\
        \btheta_{n+1} & = \btheta_n + \alpha h\bv_n  -  \beta h^2 \nabla f(\btheta_n) + \sqrt{2\gamma h}\,h \tilde\sigma \tilde\bxi_n\,,
        \label{eq:klmc}
\end{align}
where 
\begin{align}
    \alpha &= \frac{1-e^{-\gamma h}}{\gamma h} 
    \in (0,1),\qquad
    \beta =  
    \frac{e^{-\gamma h} - 1 + \gamma h  }{\gamma^2h^2}
    \in (0,1/2),\\
    \sigma^2 &=  \frac{1-e^{-2\gamma h}}{2\gamma h}\in (0,1),\qquad
    \tilde\sigma^2 =  \frac{e^{-2\gamma h} - 1 + 2\gamma h  }{2\gamma^2h^2} \in (0,1/2)
\end{align}
and $\bxi_n,\tilde\bxi_n$ are two $\mathcal N_d(\mathbf 0, \mathbf I_d)$-distributed random vectors independent
of $(\btheta_n,\bv_n)$. 


\red{To keep our main result simple and
transparent, we will without loss of generality assume $\argmin_{\btheta\in\R^d}f(\btheta)=\mathbf{0}$ and
$\min_{\btheta\in\R^d}f(\btheta)=0.$}

\begin{lemma}\textbf{[Checked by Arnak on April 10th]}
\label{lem:evmin}
Let $\mathbf{A}$, $\mathbf{B}$ and $\mathbf{C}$ be symmetric $p\times p$
matrices. If, in addition, $\mathbf{B}$ is symmetric and nonnegative definite, then
 \begin{align}
 \lambda_{\min}\bigg(\begin{bmatrix}
\hphantom{-}\mathbf{A} & -\mathbf{B} \\
-\mathbf{B} & \hphantom{-}\mathbf{C} \\
\end{bmatrix} \bigg)
\geqslant 
 \lambda_{\min}(\mathbf{A}-\mathbf{B})\wedge \lambda_{\min}(
 \mathbf{C}-\mathbf{B})\,.
 \end{align}
\end{lemma}
\begin{proof}
Consider the decomposition
\begin{align}
\begin{bmatrix}
\hphantom{-}\mathbf{A} & -\mathbf{B} \\
-\mathbf{B} & \hphantom{-}\mathbf{C} \\
\end{bmatrix}
=
\begin{bmatrix}
\mathbf{A} - \mathbf{B} & \mathbf{0} \\
\mathbf{0} & \mathbf{C} - \mathbf{B} \\
\end{bmatrix}
+
\begin{bmatrix}
\mathbf{B} & \mathbf{B} \\
\mathbf{B} & \mathbf{B}
\end{bmatrix}\,.
\end{align}
Since the eigenvalues of $\begin{bmatrix}
\mathbf{B} & \mathbf{B} \\
\mathbf{B} & \mathbf{B}
\end{bmatrix}$
are either 0 or an eigenvalue of the matrix $2\mathbf{B}$, the desired result follows readily.
\end{proof}

\begin{lemma}\textbf{[Checked by Arnak on April 10th, updated on April 15th]}
\label{lem:sum}
    Let $0 < m\leqslant M<\infty$ be two real numbers. 
    Assume that the Hessian matrix $\nabla^2 
    f(\btheta)$ of the function $f$ at any point
    $\btheta$ satisfies $m\leqslant \lambda_{\max}(\nabla^2 f(\btheta))\leqslant \lambda_{\max}(\nabla^2 f(\btheta))\leqslant M$.  
    Assume that $\bv_0$ is centered and independent of $\btheta_0$. Set 
    $\varrho = \exp(-mh/\gamma)$. 
    If the step-size $h$ and $\gamma$ satisfy $\gamma h\leqslant \gamma/(8M)$ and $\gamma^2\geqslant
    2M$, and $\bv_0=0$, then it holds for the KLMC
    iterates defined in~\eqref{eq:klmc} that
    \begin{align}
        \norm{\bv_n}_{\mathbb L_2}^2+\norm{\bv_n+\gamma(\btheta_n - \btheta^*)}_{\mathbb L_2}^2\leqslant \varrho^{n}\big(\gamma^2\norm{\btheta_0 - \btheta^*}_{\mathbb L_2}^2  + 2\|\bv_0\|_{\mathbb L_2}^2\big)+ 
        \frac{4.8\gamma^2p}{m},
    \end{align}
    where $\btheta^*: =\argmin_{ \btheta\in\R^p} 
    f(\btheta)$. 
\end{lemma}
\begin{proof}
Note that 
\begin{align}
\grad f(\btheta_n)-\grad f(\btheta^*)
=\Big[ \int_0^1 \grad^2 f(\btheta_n+u(\btheta^*-\btheta_n))du\Big](\btheta_n-\btheta^*)\,.
\end{align}
Denote the matrix $ \int_0^1 \grad^2 f(\btheta_n+u(\btheta^*-\btheta_n))\,du$ by $\bfH_n$,
and define
\begin{align}
\bz_n:=\begin{bmatrix}
\bv_n  \\
\bv_n +\gamma(\btheta_n  - \btheta^*)\\
\end{bmatrix},~~
\bfM_n:=\frac{h}{\gamma}
\begin{bmatrix}
\alpha\gamma^2\id_p -\alpha \bfH_n & \alpha \bfH_n \\
-\bfH_n & \bfH_n \\
\end{bmatrix},~~
\bzeta_n:=
\begin{bmatrix}
\sqrt{2\gamma h}\,\sigma\bxi_n\\
\sqrt{2\gamma h}\,\sigma\bxi_n
+\gamma h\sqrt{2\gamma h}\tilde\sigma\bxi_n
\end{bmatrix}\,.
\end{align}
By the definition of KLMC iterates~\eqref{eq:klmc}, we have
\begin{align}\label{zn+1}
\bz_{n+1}=(\id_{2d}-\bfM_n)\bz_n + \bzeta_n\,.
\end{align}
% We aim to show that $\norm{Z_n}_{\Lwo}^2$ is a contraction.
We aim to demonstrate the contraction property of the sequence~$\norm{\bz_n}_{\Ltwo}^2$. To this end, we 
find a suitable lower bound on $\lambda_{\min} 
(\bfM_n+\bfM_n^\top-\bfM_n^\top \bfM_n)$. Note that
\begin{align}
    \bfM_n^\top \bfM_n &= 
    \frac{h^2}{\gamma^2}
    \begin{bmatrix}
     \alpha^2\gamma^4\id_p  
     - 2\alpha^2 \gamma^2\bfH_n + (\alpha^2 + 1)\bfH_n^2
    & \alpha^2\gamma^2\bfH_n - (1+\alpha^2)\bfH_n^2\\[4pt]
    \alpha^2\gamma^2\bfH_n - (1+\alpha^2)\bfH_n^2
    & (\alpha^2+1)\bfH_n^2
\end{bmatrix}. 
\end{align}
This implies that
\begin{align}
\bfM_n+&\bfM_n^\top-\bfM_n^\top \bfM_n\\
=&\frac{h}{\gamma}\begin{bmatrix}
2\alpha ( \gamma^2 \id_p- \bfH_n)
- \frac{h}{\gamma}\big(\alpha^2\gamma^4\id_p - 2\alpha^2 \gamma^2\bfH_n + (\alpha^2+1) \bfH_n^2\big)
& 
\frac{h}{\gamma}(\alpha^2+1)\bfH_n^2
+(\alpha-1-\alpha^2\gamma h)\bfH_n
\\[8pt]
\frac{h}{\gamma}(\alpha^2 +1)\bfH_n^2
+(\alpha-1-\alpha^2\gamma h)\bfH_n
& 
2\bfH_n- \frac{h}{\gamma}(\alpha^2+1)\bfH_n^2
\end{bmatrix}\\
=&: \frac{h}{\gamma}
\begin{bmatrix}
\bfA & -\bfB\\
-\bfB & \bfC
\end{bmatrix}
\end{align}
Recall that $\alpha\in(1/2,1),$ and the eigenvalues of matrix~$\bfH_n$ fall in the interval $[m,M],$ one can verify that the eigenvalues of matrix~$\bfB$ are non negative.
Employing \Cref{lem:evmin} gives
\begin{align}\label{lmin}
\lambda_{\min}(\bfM_n+\bfM_n^\top-\bfM_n^\top \bfM_n)\geqslant (h/\gamma)\big\{
 \lambda_{\min}(\mathbf{A}+\mathbf{B})\wedge \lambda_{\min}(\mathbf{B}+\mathbf{C})\big\}.
\end{align}
We proceed by showing that $\lambda_{\min}(\mathbf{A}+\mathbf{B})\geqslant m$ and $ \lambda_{\min}
(\mathbf{B}+\mathbf{C})\geqslant m$. Note that 
\begin{align}
\bfA+\bfB
& = -\big(\alpha+1-h\alpha^2\gamma\big)\bfH_n
+2\alpha\gamma^2\id_p- h\alpha^2\gamma^3\id_p\\
& = -\big(1 + \alpha e^{-\gamma h}\big)\bfH_n + 
\alpha \gamma^2(1 + e^{-\gamma h})\id_p\\
&\succcurlyeq -\big(1 + \alpha e^{-\gamma h}\big)M\id_p + 
\alpha \gamma^2(1 + e^{-\gamma h})\id_p\\
&=  M\big(\alpha (\gamma^2/M)-1 + \alpha 
e^{-\gamma h}((\gamma^2/M)-1)\big)\id_p
\end{align}
One can check that the condition $h\leqslant \gamma/
(8M)$ implies that $\alpha \geqslant (1-e^{-z})/z$ 
with $z:= \gamma^2/(8M)\geqslant 1/2$. Therefore,
\begin{align}
    \alpha (\gamma^2/M)-1 + \alpha  e^{-\gamma h}
    ((\gamma^2/M)-1) &\geqslant 
    8(1-e^{-z})-1 + (1-e^{-z})z^{-1} e^{-z}(8z-1)\\
    &\geqslant 8(1-e^{-1/2})-1 + (1-e^{-1/2}) e^{-z}(8-2)\geqslant 2.
\end{align}
Hence, $\lambda_{\min}(\bfA + \bfB) \geqslant 2 M 
\geqslant m$.  Similarly, one can verify that 
$\bfB+\bfC=(\alpha+1-\alpha^2h\gamma)\bfH_n$ and
that $\alpha+1-\alpha^2h\gamma =   1 + \alpha 
e^{-\gamma h}\geqslant 1$.  Thus, the smallest 
eigenvalue of $\bfB+\bfC$  satisfies
\begin{align}
\lambda_{\min}(\bfB+\bfC) \geqslant m.
\end{align}
These inequalities, combined with \eqref{lmin}, 
imply that $\lambda_{\min}(\bfM_n + \bfM_n^\top + 
\bfM_n\top\bfM_n) \geqslant  mh/\gamma$. 

Going back to \eqref{zn+1}, taking the square and
the expectation, we get
\begin{align}
    \|\bz_{n+1}\|_{\mathbb L_2}^2 &\leqslant 
    (1 - mh/\gamma) \|\bz_n\|^2_{\mathbb L_2} 
    + \|\bzeta_n\|^2_{\mathbb L_2}
    \leqslant \varrho\|\bz_n\|^2_{\mathbb L_2} 
    + \|\bzeta_n\|^2_{\mathbb L_2}. 
\end{align}
One easily checks that 
\begin{align}
    \|\bzeta_n\|_{\mathbb L_2}^2 \leqslant 
    2\gamma h p \big(\sigma^2 + ( \sigma + \gamma h 
    \tilde\sigma)^2\big)
    \leqslant 2\gamma h p \big(1 + ( 1 + (\sqrt{2}/8))^2\big)   \leqslant 4.8\gamma h p. 
\end{align}
This yields 
\begin{align}
    \|\bz_{n+1}\|_{\mathbb L_2}^2 &\leqslant 
    \varrho \|\bz_n\|^2_{\mathbb L_2} 
    + 4.8 \gamma h p. 
\end{align}
Unfolding this recursive inequality, we get
\begin{align}
    \|\bz_{n}\|_{\mathbb L_2}^2 &\leqslant 
    \varrho^{n} \|\bz_0\|^2_{\mathbb L_2} 
    + 4.8 \gamma h p\times \frac{\gamma}{mh}\\
    & \leqslant \varrho^{n} \big(\gamma^2\|\btheta_0 - \btheta^*\|_{\mathbb L_2}^2 + 2\|\bv_0\|_{\mathbb L_2}^2\big) + 
    4.8\gamma^2 (p/m). 
\end{align}
This completes the proof.
\end{proof}

% \begin{theorem}
% \label{thm:klmc}
% Assume $f$ is $m$-strongly convex and $M$-smooth.
% Let the initial condition of the KLMC algorithm be drawn from the distribution $\mathcal{N}(\mathbf{0},\mathbf{I})\bigotimes \nu_0,$ and $\gamma=\sqrt{m+M}.$
% It holds for any step size $h$ satisfying  
% \begin{align}
%  h\leqslant \gamma/m \wedge \sqrt{1/(4M)}   
% \end{align} 
% that
% \begin{align}
%  W_2(\nu_n,\pi)
% \leqslant  e^{-\frac{mhn}{\gamma}} W_2(\nu_0,\pi)
% + 3.1  Mh\frac{\sqrt{d}}{m}
%  + 0.65 \gamma Mh^2 \frac{\sqrt{d}}{m}\,,
% \end{align}
% where $\nu_k$ denote the distribution of $\btheta_k$.
% \end{theorem}

% \begin{corollary}
% Assume the assumptions stated in Theorem~\ref{thm:klmc} hold, $\nu_0$ is the Dirac mass at the minimum point of $f$, and $m=1.$ 
% Given a small target precision level $\epsilon\in(0,1),$
%  for any step size
% \begin{align}
% h=\frac{\epsilon}{4M}
% \bigwedge \sqrt{\frac{\epsilon}{4M\gamma}}\,,
% \end{align}
% it holds that
% \begin{align}
%  W_2(\nu_n,\pi)\le \sqrt{d}\epsilon\,,
% \end{align}
%  provided that the number of iterations
% \begin{align}
% n \geqslant 
% \frac{4\gamma M}{\epsilon}\log\Big(\frac{2}{\epsilon}\Big)
% \bigvee
% \gamma\sqrt{\frac{4\gamma M}{\epsilon}}\log\Big(\frac{2}{\epsilon}\Big)
%  \,.
% \end{align}

% \end{corollary}

% \begin{proof}[Proof of~\Cref{thm:klmc}]
% Let $\btheta_n,\bv_n$ be the iterates of KLMC algorithm.
% Let $(\tilde\btheta_n,\tilde\bv_n)$ be the $n$-th step of the exact underdamped Langevin diffusion, coupled with $(\btheta_n,\bv_n)$ through the same Brownian motion and starting from a random point $(\tilde\btheta_0,\tilde\bv_0)\propto \exp(-f(\btheta)+\frac{1}{2}\norm{\bv}^2)$ such that $\tilde \bv_0=\bv_0$. 
% Let $(\btheta_{n+1}^*,\bv_{n+1}^*)$ be the 1-step exact Langevin diffusion starting from $(\btheta_n,\bv_n).$

% Set $A_n := \EE^{1/2}\Big[\norm{\bv_n-\tilde\bv_n 
% + \gamma \btheta_{n}-\gamma \tilde\btheta_n}^2 + 
% \norm{ \bv_n-\tilde\bv_{n}}^2 \Big]$. The triangle inequality for the
% $\mathbb L_2$-norm implies that
% \begin{align}
% A_{n+1} &\leqslant \E^{1/2}\Big[\norm{\tilde\bv_{n+1}+\gamma\tilde\btheta_{n+1}-\bv_{n+1}^*-\gamma\btheta_{n+1}^*}^2+\norm{\tilde\bv_{n+1}-\bv_{n+1}^*}^2\Big]  \\
%     &\qquad +  \EE^{1/2}\Big[\| \bv_{n+1}^* + \gamma \btheta_{n+1}^* -
%     \bv_{n+1} - \gamma \btheta_{n+1} \|^2 + \| \bv_{n+1}^* 
%     - \bv_{n+1}\|^2\Big]\\
%     &\leqslant  e^{-mh/\gamma} A_n + \sqrt{2}\norm{\bv_{n+1}^* - \bv_{n+1}}_{\Ltwo} + \gamma 
%     \norm{ \btheta_{n+1}^* - \btheta_{n+1}}_{\Ltwo}\,.
% \end{align}
% The last step follows from the proof of Proposition 1 in \citep{dalalyan_riou_2018} 
%  by choosing $\gamma^2 = m+M$, 
% $\lambda_+ = \gamma$, $\lambda_- =0.$
% One can check by induction, that if for some sequences $A_n,B_n$ and some $\varrho \in(0,1)$ it holds that $A_n\leqslant B_n + \varrho A_{n-1}$, then necessarily 
% $A_n\leqslant \varrho^n A_0 + 
% \sum_{k=1}^n \varrho^{n-k}B_k$.
% Hence,
% \begin{align}
% A_{n} &\leqslant 
%  e^{-\frac{mhn}{\gamma}} A_0 
%  + \sum_{k=1}^n e^{-\frac{mh(n-k)}{\gamma}}
%  \Big\{\sqrt{2}\norm{\bv_{k}^* - \bv_{k}}_{\Ltwo} + \gamma 
%     \norm{ \btheta_{k}^* - \btheta_{k}}_{\Ltwo}
% \Big\}\,.
% \end{align}
% By Lemma~\ref{lem:klmc} and the fact that $\norm{\bv_k}_{\Ltwo}=\sqrt{d}$ and $\norm{\grad f(\btheta_k)}_{\Ltwo}\leqslant\sqrt{dM}$, when $Mh^2\leqslant 1/4,$ it holds that
% \begin{align}
% \sqrt{2}\sum_{k=1}^n e^{-\frac{mh(n-k)}{\gamma}}
% \norm{\bv_{k}^* - \bv_{k}}_{\Ltwo}
% &\leqslant \sqrt{2} \sum_{k=0}^{n-1} e^{-\frac{mh(n-k)}{\gamma}} 0.5Mh^2e^{\frac{Mh^2}{2}}\Big(0.8\sqrt{\gamma d h}
% +\norm{\bv_{k}}_{\Ltwo}
% +0.4 h\norm{\grad f(\btheta_k)}_{\Ltwo}
% \Big) \\
% &\leqslant  1.52 Mh^2\sqrt{d} \sum_{k=0}^{n-1} e^{-\frac{mh(n-k)}{\gamma}}  \\
% &\leqslant 3.1 \gamma Mh\frac{\sqrt{d}}{m}\,,
% \end{align}
% where the last inequality follows from 
% \begin{align}
% \sum_{k=0}^{n-1}e^{-\frac{mh(n-k)}{\gamma}}
% \leqslant
% \frac{1}{1-e^{-\frac{mh}{\gamma}}}
% \leqslant \frac{2\gamma}{mh}
% \end{align}
% given that $\frac{mh}{\gamma}\leqslant 1.$
% Similarly, we have
% \begin{align}
%  \gamma \sum_{k=1}^n e^{-\frac{mh(n-k)}{\gamma}}
%     \norm{ \btheta_{k}^* - \btheta_{k}}_{\Ltwo}
% &\leqslant \gamma \sum_{k=0}^{n-1} e^{-\frac{mh(n-k)}{\gamma}} \frac{1}{6}Mh^3 e^{Mh^2/2} \big(0.7\sqrt{\gamma dh} 
% + \|\bv_n\|_{\mathbb L_2}
% + 0.25h\norm{\grad f(\btheta_k)}_{\Ltwo} \big) \\
% &\leqslant 0.65 \gamma^2Mh^2 \frac{\sqrt{d}}{m} \,.
% \end{align}
% Collecting pieces then gives
% \begin{align}
% A_{n} &\leqslant 
%  e^{-\frac{mhn}{\gamma}} A_0 
%  +  3.1 \gamma Mh\frac{\sqrt{d}}{m}
%  + 0.65 \gamma^2Mh^2 \frac{\sqrt{d}}{m}\,.
% \end{align}
% It follows that
% \begin{align}
% W_2(\nu_n,\pi)
% \leqslant  e^{-\frac{mhn}{\gamma}} W_2(\nu_0,\pi)
% + 3.1  Mh\frac{\sqrt{d}}{m}
%  + 0.65 \gamma Mh^2 \frac{\sqrt{d}}{m}
% \end{align}
% as desired.

% \end{proof}

%\newpage
%{\color{blue}


%I guess that there is a relatively simple way
%to upper bound the sums $\sum_{k=0}^n \|\bv_k\|^2$
%and $\sum_{k=0}^n \|\nabla f(\bvartheta_k)\|^2$ 
%by an expression of the order of $n$. The explanations
%are below. 



%\begin{lemma}
%    Let $\rho_1 = 1 - (11/15)mh^2$.
%    For $\gamma^2 = m+M $ and for $\gamma h \leqslant 1/4$,
%    it holds that 
%    \begin{align}
%        \E[f(\btheta_n)] 
%        &\leqslant \rho_1^{n}
%        \E[ f(\btheta_0)] + 
%        h\sum_{k=1}^{n}
%        \rho_1^{n-k}
%        \E_+[\nabla f(\btheta_{k-1})^\top\bv_{k-1}] 
%        +\frac{Mh^2}{2}\sum_{k=1}^{n} \rho_1^{n-k}
%        \E[\|\bv_{k-1}\|^2] + \frac{15M h\gamma d}{22m},\\
%        h^2\E[\| \nabla f(\btheta_n)\|^2] 
%        &\leqslant 3 h\E_+[\nabla f(\btheta_n)^\top\bv_n] +{1.4 Mh^2}
%        \E[\|\bv_n\|^2] + {0.4 \gamma d h}
%        +2.8\E[f(\btheta_n)]\\
%        &\leqslant 2.8\rho_1^n \E[f(\btheta_0)] + 3 h\sum_{k=0}^{n}
%        \rho_1^{n-k}\E_+[\nabla f(\btheta_{k})^\top\bv_{k}] 
%        + {1.5 Mh^2}\sum_{k=0}^{n}
%        \rho_1^{n-k} \E[\|\bv_{k}\|^2] + {2.4 \kappa h\gamma d}.
%    \end{align}
%    for every $n\in\mathbb N$.
%\end{lemma}
%
%\begin{proof}
%    Using the Lipschitz-gradient property, one can check that 
%    \begin{align}
%        \E[f(\btheta_{n+1}) -f(\btheta_n)] 
%        &\leqslant \alpha h(1 -  M \beta h^2)\E[\nabla f(\btheta_n)^\top\bv_n] - \frac{\beta h^2}{2}(2 -M\beta h^2) \E[\| \nabla f(\btheta_n)\|^2] \\
%        &\qquad+\frac{M\alpha^2 h^2}{2}
%        \E[\|\bv_n\|^2] + M \gamma \tilde\sigma^2 d h^3\\
%        &\leqslant \alpha h(1 - \beta Mh^2)\E[\nabla f(\btheta_n)^\top\bv_n] - \frac{11h^2}{30} 
%        \E[\| \nabla f(\btheta_n)\|^2] +\frac{Mh^2}{2}
%        \E[\|\bv_n\|^2] + \frac{M\gamma d h^3}{2}
%        \label{eq:df}
%    \end{align}
%    where we have used the fact that
%    \begin{align}
%        2\beta - M\beta^2 h^2 &\geqslant 2\beta -
%        (M/4) h^2 \geqslant 0.8 - 1/16 \geqslant 11/15.
%    \end{align}
%    It is well-known that for any $m$-strongly convex function $f$ and for any point $\btheta$, it holds that $\|\nabla f(\btheta)\|^2\geqslant 2m(f(\btheta)-f_*) = 2mf(\btheta)$. This fact, combined with the last display, 
%    implies that
%    \begin{align}
%        \E[f(\btheta_{n+1})]   
%        &\leqslant \Big(1 -\frac{11 mh^2}{15} \Big)
%        \E[ f(\btheta_n)] + 
%        \alpha h(1 - \beta Mh^2)\E[\nabla f(\btheta_n)^\top\bv_n]  +\frac{Mh^2}{2}
%        \E[\|\bv_n\|^2] + \frac{M\gamma dh^3}{2}.
%    \end{align}
%    Thus, setting $\rho_1 = 1 - (11/15)mh^2\geqslant 
%    0.8$ and 
%    unfolding this recursive inequality, we get 
%    \begin{align}
%        \E[f(\btheta_{n+1})]   
%        &\leqslant \rho_1^{n+1}
%        \E[ f(\btheta_0)] + 
%        \alpha h(1 - \beta Mh^2)\sum_{k=0}^n\rho_1^{n-k}
%        \E[\nabla f(\btheta_k)^\top\bv_k] +\frac{Mh^2}{2}\sum_{k=0}^n \rho_1^{n-k}
%        \E[\|\bv_k\|^2] + \frac{15M h\gamma d}{22m}.
%    \end{align}
%    One can also infer from \eqref{eq:df} that
%    \begin{align}
%        \frac{11h^2}{30} 
%        \E[\| \nabla f(\btheta_n)\|^2] 
%        &\leqslant \alpha h(1 - \beta Mh^2)\E[\nabla f(\btheta_n)^\top\bv_n] +\frac{Mh^2}{2}
%        \E[\|\bv_n\|^2] + \frac{M\gamma d h^3}{2}
%        +\E[f(\btheta_n)]
%        %\\&\leqslant \rho_1^{n} \E[ f(\btheta_0)] + 
%        %\frac{\alpha h(1 - \beta Mh^2)}{\rho_1}\sum_{k=0}^n\rho_1^{n-k}
%        %\E[\nabla f(\btheta_k)^\top\bv_k] +\frac{Mh^2}{2}\sum_{k=0}^n \rho_1^{n-k}
%        %\E[\|\bv_k\|^2] + \frac{9Mh\gamma d}{11m}
%        .
%    \end{align}
%    This completes the proof of the lemma.
%\end{proof}


\begin{lemma} \textbf{[Checked by Arnak on April 15th]}
\label{lem:inprod}
    If for some $M\geqslant 0$, the gradient $\nabla f$ 
    is $M$-Lipschitz continuous, then for every 
    step-size $h>0$ and every $\gamma>0$ it holds for the KLMC
    iterates defined in~\eqref{eq:klmc} that 
\begin{align}
         \E[\nabla f(\btheta_{n+1})^\top \bv_{n+1}]
        &\leqslant (1-\alpha \gamma h)  \E[\nabla f(\btheta_n)^\top \bv_n] + 
        3Mh\|\bv_n\|_{\mathbb L_2}^2 + 6M\gamma h^2p -  h (\alpha - 3Mh^2)\E[\|\nabla f(\btheta_n)\|^2].
        %\label{eq:Zn}
    \end{align}
\end{lemma}

\begin{proof}
To ease notation, let us set $\nabla f_n = \nabla f(\btheta_n)$.  By the definitions of 
$\btheta_{n+1}$ and $\bv_{n+1},$ it holds that 
    \begin{align}
        \E[\nabla f_{n+1}^\top \bv_{n+1}] -\E[\nabla f_n^\top \bv_n] &= \E\big[\big(\nabla f_{n+1} - \nabla f_n\big)^\top \bv_{n+1} ] + \E[\nabla f_n^\top (\bv_{n+1} -\bv_n)]\\
        &\leqslant \big\|\nabla f_{n+1} - \nabla f_n\big\|_{\mathbb L_2}\|\bv_{n+1}\|_{\mathbb L_2} + \E[\nabla f_n^\top (\bv_{n+1} -\bv_n)]\\
        & = M\|\btheta_{n+1} - \btheta_n\|_{\mathbb L_2}\|\bv_{n+1}\|_{\mathbb L_2}-\alpha\gamma h \E[\nabla f_n^\top \bv_n]-\alpha h \|\nabla f_n\|_{\mathbb L_2}^2. 
    \end{align}
    Similar arguments yield
    \begin{align}
        \|\btheta_{n+1} - \btheta_n\|_{\mathbb L_2}
        &\leqslant  h\|\bv_n\|_{\mathbb L_2} + 
        (1/2)h^2 \|\nabla f_n\|_{\mathbb L_2} + 
        h\sqrt{\gamma h p}\\
        \|\bv_{n+1}\|_{\mathbb L_2}&\leqslant 
        \|\bv_n\|_{\mathbb L_2} + h\|\nabla f_n\|_{\mathbb L_2} + \sqrt{2\gamma hp}.
    \end{align}
    This implies that
    \begin{align}
        \|\btheta_{n+1} - \btheta_n\|_{\mathbb L_2}
        \|\bv_{n+1}\|_{\mathbb L_2}
        &\leqslant  3h\|\bv_n\|_{\mathbb L_2}^2 + 
        3h^3 \|\nabla f_n\|_{\mathbb L_2}^2 + 
        3h^2\gamma p.
    \end{align}
    Therefore, we get
    \begin{align}
        \E[\nabla f_{n+1}^\top \bv_{n+1}] 
        &\leqslant (1-\alpha \gamma h)\E[\nabla f_n^\top \bv_n] + 
        3Mh\|\bv_n\|_{\mathbb L_2}^2 + 6M\gamma h^2p -  h (\alpha - 3Mh^2)\E[\|\nabla f_n\|^2]
    \end{align}
    as desired.
%    Using the fact that the last term is negative and
%    unfolding the obtained recursive inequality, we get
%    \begin{align}
%        Z_{n+1} &\leqslant (1-\rho_2)^{n+1} Z_0 + 
%        3Mh\sum_{k=0}^n \rho_2^{n-k} \|\bv_k
%        \|_{\mathbb L_2}^2 + 3Mhd/\alpha.
%    \end{align}
%    Using the facts that $Z_0 = 0$ and $\alpha\geqslant 
%    0.7$, we get the first claim of the lemma.
\end{proof}

%\begin{lemma}
%    For $\gamma^2 = m + M$ and $\gamma h\leqslant 1/4$, 
%    it holds that 
%    \begin{align}
%        \E[\|\bv_n\|^2]
%        \leqslant 
%    \end{align}
%\end{lemma}
%
%\begin{proof}
%Define the sequence
%\begin{align}
%    z_n = \E\Big[ f(\btheta_n) + \frac{1 - M \beta h^2} {2(1-\alpha\gamma h)}\|\bv_n\|^2\Big].
%\end{align}
%Applying the formulae  \eqref{vn1} and \eqref{thn1} for computing
%$z_{n+1}$, one can check that the cross term $\E[\nabla f(\btheta_n)^\top \bv_n]$ cancels out and we get
%\begin{align}
%    z_{n+1} - z_n & \leqslant 2Mh^3\gamma \sigma^2 d  
%    + \frac{\gamma h \tilde\sigma^2 d}{1-\alpha \gamma h}
%    - \frac12\big(2\gamma h \sigma^2 (1-M\beta h^2) - M\alpha^2 h^2\big)\E[\|\bv_n\|^2]\\
%    &\qquad-\frac{h^2}{2(1-\alpha \gamma h)} 
%    \big\{(2\beta - M\beta^2 h^2)(1-\alpha \gamma h)- \alpha^2(1 - M\beta h^2)\big\}\E[\|\nabla f(\btheta_n)\|^2]\\
%    &\leqslant 2Mh^3\gamma d  
%    + \frac{2\gamma h d}{3}
%    - \frac12\big(\gamma h \sigma^2 (2-M h^2) - M h^2\big)\E[\|\bv_n\|^2] \\
%    &\qquad + \frac{2h^2}{3} 
%    \big\{\alpha^2 + \gamma h + (M/4) h^2 - 2\beta\big\}\E[\|\nabla f(\btheta_n)\|^2].
%\end{align}
%In addition, if we use the value $\gamma = \sqrt{m + M}$,
%we get
%\begin{align}
%    z_{n+1} - z_n 
%    &\leqslant \frac56 \gamma h d  
%    - \frac{( 31\sigma^2  - 4)\gamma h}{32}\E[\|\bv_n\|^2] +
%    \frac{2\gamma h^3}{3} 
%    \Big\{\frac{1-2\beta}{\gamma h} + \frac{17}{16}\Big\}\E[\|\nabla f(\btheta_n)\|^2].
%\end{align}
%Note that 
%\begin{align}
%    \frac{1-2\beta}{\gamma h} &= -\frac{ e^{-\gamma h} -1 +\gamma h - \frac12 (\gamma h)^2}{(\gamma h)^3}\leqslant -0.15,\qquad \text{for}\qquad 
%    \gamma h \in (0,1/4],\\
%    \sigma^2 &=  \frac{1-e^{-2\gamma h}}{2\gamma h} \geqslant 0.78
%\end{align}
%This implies that 
%\begin{align}
%    z_{n+1} - z_n 
%    &\leqslant \frac56 \gamma h d  
%    - \frac{3\gamma h}{5}\E[\|\bv_n\|^2] +
%    \frac{2\gamma h^3}{3} \E[\|\nabla f(\btheta_n)\|^2].
%\end{align}
%Hence, by replacing $z_n$ with its expression, we arrive at
%\begin{align}
%    \frac{1-M\beta h^2}{2(1-\alpha \gamma h)} \,\E[\|\bv_{n+1}\|^2]
%    &\leqslant \Big(\frac{1-M\beta h^2}{2(1-\alpha \gamma h)} -
%    \frac{3\gamma h}{5}\Big)\,\E[\|\bv_{n}\|^2]  + 
%    \frac56 \gamma h d  +
%    \frac{2\gamma h^3}{3} \E[\|\nabla f(\btheta_n)\|^2]
%    +\E[f(\btheta_n) - f(\btheta_{n+1})].\label{eq:vn2}
%\end{align}
%Since 
%\begin{align}
%   \frac{3}{2} \leqslant \mathfrak C : =
%   \frac{2(1-\alpha \gamma h)}{1-M\beta h^2} \leqslant 
%    \frac{64}{31},
%\end{align}
%equation \eqref{eq:vn2} yields
%\begin{align}
%    \E[\|\bv_{n+1}\|^2]
%    &\leqslant \Big(1 - 
%    \frac{9\gamma h}{10}\Big)\,\E[\|\bv_{n}\|^2]  + 
%    \frac{16}{9} \gamma h d  + 
%    \frac{7\gamma h^3}{5} \E[\|\nabla f(\btheta_n)\|^2]
%    +\mathfrak C\E[f(\btheta_n) - f(\btheta_{n+1})].\label{eq:vn2}
%\end{align}
%Recall that $\rho_3 = 1-0.9 \gamma h $. If we unfold the 
%inequality of the last display, we get
%\begin{align}
%    \E[\|\bv_{n+1}\|^2]
%    &\leqslant \rho_3^{n+1}\,\E[\|\bv_{0}\|^2]  + 
%    \frac{160 d}{81}   + 
%    \frac{7\gamma h^3}{5} \sum_{k=0}^n \rho_3^{n-k}\E[\|\nabla f(\btheta_k)\|^2]
%    +\mathfrak C \sum_{k=0}^n \rho_3^{n-k}\E[f(\btheta_k) - f(\btheta_{k+1})]\\
%    &\leqslant 
%    \frac{160 d}{81}   + 
%    \frac{7\gamma h^3}{5} \sum_{k=0}^n \rho_3^{n-k}\E[\|\nabla f(\btheta_k)\|^2] + \mathfrak C \rho_3^n\E[f(\btheta_0)]
%    + 0.9\mathfrak C \gamma h\sum_{k=1}^n \rho_3^{n-k}\E[f(\btheta_k)]. 
%\end{align}
%\end{proof}

\begin{proposition}
\label{lem:sum2} \textbf{[Checked by Arnak on April 14th]}
Set $\varrho = \exp(-mh/\gamma)$. Assume that $\E[\bv_0] = 0$  and $\bv_0$ is independent of $\btheta_0$. If $\gamma^2\geqslant 2M$ and 
$h\leqslant \gamma/(8M)$ then
\begin{align}
    \sum_{k=0}^{n}  \varrho^{n - k} (\|\bv_k\|_{\mathbb L_2}^2  + 7 h^2 
     \|\nabla f(\btheta_k)\|_{\mathbb L_2}^2)
    \leqslant \frac{18.4 \gamma}{h}\Big\{\frac{ p}{m} + 
    \rho^n \big(\|\btheta_0-\btheta^*\|_{\mathbb L_2}^2 +  \gamma^{-2}\|\bv_0\|_{\mathbb L_2}^2 \big)\Big\}.
\end{align}
\end{proposition}


\begin{proof}
To ease notation, let us set $f_n = f(\btheta_n)$ and 
$\nabla f_n = \nabla f(\btheta_n)$.
Define the sequence
\begin{align}
    Y_n := \E\Big[2f_n + \|\bv_n\|^2 + 
    2h\big(\alpha  - (M/\gamma)\beta h\big) \nabla f_n^\top \bv_n\Big]. 
\end{align}
Using the Lipschitz-gradient property, one can check that 
    \begin{align}
        2\E[f_{n+1} -f_n] 
        &\leqslant 2\alpha h(1 -  M \beta h^2)\E[\nabla f_n^\top\bv_n] - {\beta h^2}(2 -M\beta h^2) \| \nabla f_n\|^2_{\mathbb L_2} 
        + {M\alpha^2 h^2}
        \|\bv_n\|^2_{\mathbb L_2} + 2\tilde\sigma^2{M 
        \gamma p h^3}.
        \label{eq:df}
    \end{align}
By the definition of $\bv_n$,  we have
\begin{align}
    \|\bv_{n+1}\|_{\mathbb L_2}^2 - \|\bv_n\|_{\mathbb L_2}^2 &\leqslant 
    -\alpha\gamma h(2-\alpha \gamma h) \|\bv_n\|^2_{\mathbb L_2} 
    -2\alpha h(1-\alpha \gamma h)\E[\nabla f_n^\top 
    \bv_n] + (\alpha h)^2\|\nabla f_n\|_{\mathbb L_2}^2 + 2\sigma^2\gamma p h.
\end{align}
Finally, by ~\Cref{lem:inprod}, we find
\begin{align}
    \E[\nabla f_{n+1}^\top\bv_{n+1} - 
    \nabla f_n^\top\bv_n] 
    &\leqslant -\alpha \gamma h \E[
    \nabla f_n^\top\bv_n]  + 
    3Mh\|\bv_n\|_{\mathbb L_2}^2 + 6M\gamma p h^2 -  h (\alpha - 3Mh^2)\|\nabla f_n\|^2_{\mathbb L_2}.
\end{align}
Collecting the pieces provides us with the following inequality
\begin{align}
    Y_{n+1} - Y_n &\leqslant \Big\{ M\alpha^2 h^2 
 - \alpha\gamma h (2 - \alpha\gamma h) +6Mh^2\big(\alpha - (M/\gamma)\beta h\big)\Big\}\|\bv_n\|_{\mathbb L_2}^2\\
 &\qquad - \Big\{ \beta h^2(2 - M\beta h^2) 
 - (\alpha h)^2 +2h^2\big(\alpha - (M/\gamma)\beta h\big)
 (\alpha - 3Mh^2)\Big\}\|\nabla f_n\|_{\mathbb L_2}^2\\
 &\qquad + \gamma p h (M h^2 + 2 + 12Mh^2),
\end{align}
where the last term has been simplified using the fact
that $\alpha - (M/\gamma)\beta h\leqslant 1$. 
Using conditions $\gamma^2\geqslant 2M$ and 
$h\leqslant \gamma/(8M)$ (this implies that 
$\beta\geqslant 0.46$ and $\alpha\geqslant 0.88$), one can deduce from the
last display the following simpler inequality
\begin{align}
    Y_{n+1} - Y_n &\leqslant - 0.63\gamma h \|\bv_n\|_{\mathbb L_2}^2 - 1.18h^2\|\nabla f_n\|_{\mathbb L_2}^2+ (2 + 13 Mh^2)\gamma p h .
\end{align}
Rearranging the inequality gives
\begin{align}
    0.63 \|\bv_n\|_{\mathbb L_2}^2 + 1.18 (h/\gamma) 
    \|\nabla f_n\|_{\mathbb L_2}^2
    \leqslant 2.5 p + \frac{Y_n-Y_{n+1}}{\gamma h}.
\end{align}
As a consequence, we obtain
\begin{align}
    0.6\sum_{k=0}^{n} \varrho^{n-k}\big(\|\bv_k\|_{\mathbb L_2}^2 + 7 h^2
    \|\nabla f_k\|_{\mathbb L_2}^2\big)
    &\leqslant \frac{2.5  \gamma p}{mh} + 
    \sum_{k=0}^{n} \varrho^{n - k} 
    \frac{Y_k-Y_{k+1}}{\gamma h}\\
    &\leqslant \frac{2.5 \gamma p}{mh} + 
    \varrho^{n}\frac{Y_0}{\gamma h}
    -\frac{Y_{n+1}}{\gamma h}
    + 
    (1-\varrho)\sum_{k=1}^{n} \varrho^{n - k}\frac{|Y_k|}{\gamma h}.\label{eq:18}
\end{align}
On the one hand, since $\bv_0$ is centered and independent
of $\btheta_0$, we have $Y_0 = 2\E[f_0] + 
\|\bv_0\|_{\mathbb L_2}^2 \leqslant M\|\btheta_0 -\btheta^*\|_{\mathbb L_2}^2 + \|\bv_0\|_{\mathbb L_2}^2 \leqslant 0.5
(\gamma^2\|\btheta_0 -\btheta^*\|_{\mathbb L_2}^2 + 2\|\bv_0\|_{\mathbb L_2}^2)$. On the other hand, $2f_k \leqslant 2f(\btheta^*) + 
2\nabla f (\btheta^*)^\top(\btheta_k-\btheta^*) + M\|\btheta_k-\btheta^*\|^2 = 
M\|\btheta_k-\btheta^*\|^2$ and
\begin{align}
    \Big|2h\big(\alpha-(M/\gamma)\beta h\big) \nabla f_k^\top \bv_k\Big|&\leqslant 2h\|\nabla f_k\| 
    \|\bv_k\|\leqslant 2Mh\|\btheta_k - \btheta^*\|\,\|\bv_k\|\\
    &\leqslant \sqrt{M}h\big(M\|\btheta_k - \btheta^*\|^2 + \|\bv_k\|^2\big)
    \leqslant 0.09 \big(\gamma^2\|\btheta_k - \btheta^*\|^2 + 2\|\bv_k\|^2\big);
\end{align}
these inequalities together yield $-Y_{n+1}\leqslant 0.09 \big(\gamma^2\|\btheta_n - \btheta^*\|^2 + 2\|\bv_n\|^2\big) $ and 
$ |Y_k|\leqslant 0.59\big(\gamma^2\|\btheta_k - \btheta^*\|^2 + 2\|\bv_k\|^2\big) $. 
Furthermore,  
one can check that $\gamma^2\|\btheta_k -\btheta^*\|^2 + 
2\|\bv_k\|^2 \leqslant 3.41\big\{\|\bv_k\|^2 + \|\bv_k + \gamma (\btheta_k-\btheta^*)\|^2\big\}$. Therefore, in view of \Cref{lem:sum},
\begin{align}
    -Y_{n+1} &\leqslant 0.31\big\{\|\bv_k\|^2 + \|\bv_k + \gamma (\btheta_k-\btheta^*)\|^2\big\}\leqslant
    0.31\varrho^{n}\big(\gamma^2\|\btheta_0-\btheta^*\|^2_{\mathbb L_2} +\|\bv_0\|^2_{\mathbb L_2}\big) + 1.5\gamma^2 p/m\\
    |Y_k|&\leqslant 2.02\big\{\|\bv_k\|^2 + \|\bv_k + \gamma (\btheta_k-\btheta^*)\|^2\big\}
    \leqslant  2.02\varrho^{k}\big(\gamma^2\|\btheta_0-\btheta^*\|^2_{\mathbb L_2} +\|\bv_0\|^2_{\mathbb L_2}\big)  + 9.7\gamma^2 p/m.
\end{align}
Combining these inequalities with \eqref{eq:18}, we get 
\begin{align}
    \sum_{k=0}^{n}  \varrho^{n - k} (\|\bv_k\|_{\mathbb L_2}^2  + 7 h^2 
     \|\nabla f(\btheta_k)\|_{\mathbb L_2}^2)
    &\leqslant \frac{18.4 \gamma p}{mh} + 
    \rho^n \frac{12\gamma^2\|\btheta_0-\btheta^*\|_{\mathbb L_2}^2 +  13 
    \|\bv_0\|_{\mathbb L_2}^2 }{\gamma h}\\
    &\leqslant \frac{18.4 \gamma}{h}\Big\{
    \frac{ p}{m} + 
    \rho^n \big(\|\btheta_0-\btheta^*\|_{\mathbb L_2}^2 +  \gamma^{-2}\|\bv_0\|_{\mathbb L_2}^2 \big)\Big\}
\end{align}
and the claim of the proposition follows.
\end{proof}



%\begin{lemma}
%    Let $(a_k)_{k\geqslant 0}$ be a sequence of positive
%    numbers such that $\bar a = \max_{n\geqslant 1}
%    \frac1n \sum_{k=0}^{n-1} a_k <\infty$. For
%    any $\rho<1$, we have
%    \begin{align}
%        \sum_{k=0}^n \rho^{n-k} a_k \leqslant 
%    \end{align}
%\end{lemma}
%\begin{proof}
%    Let us set $S_k = \sum_{j=0}^k a_j$. 
%    Simple algebra yields
%    \begin{align}
%        \sum_{k=0}^n \rho^{n-k} a_k & = 
%        \sum_{k=0}^n \rho^{n-k} S_k - \sum_{k=1}^n \rho^{n-k} S_{k-1}
%        = \sum_{k=0}^n \rho^{n-k} S_k - \sum_{k=0}^{n-1} \rho^{n-1-k} S_{k}
%    \end{align}
%\end{proof}
%}

%\begin{lemma}
%\label{lem:klmc1}
%Let $\{v_n(t),\theta_n(t)\}$ be the solution of SDE starting from $(v_n,\theta_n),$
% and let $(v_n,\theta_n)$ be the starting point at the $n$-th iteration of the algorithm.
%When $Lh^2\leqslant 0.001,$ we have
% \begin{align}
%\E [f(\theta_{n+1}(0))
%- f(\theta_n(h))]
%\leqslant
% 0.183 h^2 \norm{\grad f(\theta_n)}^2_{\Ltwo}
%+ 0.58 M^{2}h^4 \norm{v_n}^{2}_{\Ltwo}
%+0.34 M^{2}h^5\gamma d\,.
% \end{align}
%\end{lemma}
%\begin{proof}
%By Taylor expansion and Young's inequality, we have
%\begin{align}
%f(\theta_{n+1}(0))
%& \leqslant f(\theta_n(h))
%+\grad f(\theta_n(h))^\top(\theta_{n+1}(0)-\theta_n(h))
%+\frac{M}{2}\norm{\theta_{n+1}(0)-\theta_n(h)}^2\\
%& \leqslant  f(\theta_n(h))
%+ \frac{10}{2h^2}\norm{\theta_{n+1}(0)-\theta_n(h)}^2
%+\frac{h^2}{20}\norm{\grad f(\theta_n(h)}^2
%+\frac{M}{2}\norm{\theta_{n+1}(0)-\theta_n(h)}^2
%\end{align}
%By Lemma~\ref{lem:6}, Lemma~\ref{lem:klmc}, and $Lh^2\leqslant 0.001,$ we have
%\begin{align}
%\E[f(\theta_{n+1}(0))
%-f(\theta_n(h))]
%&\leqslant \frac{h^2}{20}(3.07\norm{f(\theta_n)}_{\Ltwo}^2
%+3.07M^2h^2\norm{v_n}^2_{\Ltwo}
%+2.7M^2h^3\gamma d) \\
%&\quad + \frac{5}{h^2} \frac{M^2h^6}{12}( 0.25^2h^2\norm{f(\theta_n)}_{\Ltwo}^2
%+\norm{v_n}^2_{\Ltwo}
%+0.49\gamma dh)  \\
%&\quad + \frac{M}{2}
%\frac{M^2h^6}{12}( 0.25^2h^2\norm{f(\theta_n)}_{\Ltwo}^2
%+\norm{v_n}^2_{\Ltwo}
%+0.49\gamma dh) \\
%&\leqslant 0.183 h^2 \norm{\grad f(\theta_n)}^2_{\Ltwo}
%+ 0.58 M^{2}h^4 \norm{v_n}^{2}_{\Ltwo}
%+0.34 M^{2}h^5\gamma d\,.
%\end{align}
%
%\end{proof}


%\begin{lemma}
%\label{lem:11_klmc}
%Set $(v_n,x_n)$ as the initialization of the algorithm at $n$-th iteration.
%Denote the solution of the exact underdamped Langevin diffusion starting from $(v_n,x_n)$ by $(v_n(t),x_n(t)).$
%Assume $h\leqslant \sqrt{1/(1000L)}\wedge \gamma/m$ and $\gamma^2=L+m.$
%It holds that
%% \begin{align}
%% \sum_{k=0}^{n-1}e^{-\frac{mh(n-k)}{\gamma}}\norm{v_k(0)}^2_{\Ltwo}
%% \leqslant 0.59 \frac{h}{\gamma}\sum_{k=0}^{n-1}e^{-\frac{mh(n-k)}{\gamma}} \norm{\grad f(x_k(0))}^2_{\Ltwo} 
%% +8.12\frac{d\gamma}{mh}\,.
%% \end{align}
%\begin{align}
%\sum_{k=0}^{n-1}\norm{v_k(0)}_{\Ltwo}^2
%& \leqslant 
%0.59\frac{h}{\gamma} \sum_{k=0}^{n-1} \norm{\grad f(x_k(0))}^2_{\Ltwo} 
%+ 4.06dn  \,.
%\end{align}
%
%\end{lemma}
%\begin{proof}
%By It\^{o}'s lemma and the definition of $(v_n(t),x_n(t)),$ we have
%\begin{align}
%df(x_n(t))=\grad f(x_n(t))^\top v_n(t),\quad t\in[0,h]\,.
%\end{align}
%This implies
%\begin{align}
%f(x_n(h))
%=&f(x_n(0))+\int_0^hdf(x_n(t))\\
%=&f(x_n(0))+\int_0^h\grad f(x_n(t))^\top v_n(t)dt\,.
%\end{align}
%Moreover, we have
%\begin{align}
%dv_n(t)=\big(-\gamma v_n(t)-\grad f(x_n(t))\big)dt+\sqrt{2\gamma} dB_t\,.
%\end{align}
%Using It\^{o}'s lemma again, we obtain
%\begin{align}
%d\frac{1}{2}\norm{v_n(t)}^2
%= \sqrt{2\gamma}v_n(t)^\top dB_t
%+ \big(-\gamma\norm{v_n(t)}^2-v_n(t)^\top\grad f(x_n(t))+\gamma d\big)dt
%\end{align}
%which implies
%\begin{align}
%\E\frac{1}{2}\norm{v_n(h)}^2
%=\E\frac{1}{2}\norm{v_n(0)}^2
%+\E\int_0^h \big(2d\gamma-\gamma\norm{v_n(t)}^2-v_n(t)^\top\grad f(x_n(t))+\gamma d\big)dt\,.
%\end{align}
%Then, we have
%\begin{align}
%\E\Big[\frac{1}{2}\norm{v_n(h)}^2+f(x_n(h))\Big]
%= & \E\Big[\frac{1}{2}\norm{v_n(0)}^2
%+ f(x_n(0))
%- \gamma  \int_0^h \norm{v_n(t)}^2dt +3\gamma d h\Big]\,.
%\end{align}
%Invoking~\Cref{lem:6} and by the fact that $\gamma^2 =L+m, Lh^2\leqslant 0.001,$ we then obtain
%\begin{align}
%\E\Big[\frac{1}{2}&\norm{v_n(h)}^2 +f(x_n(h))\Big]\\
%& \leqslant \E\Big[\frac{1}{2}\norm{v_n(0)}^2+f(x_n(0))\Big]
%+\gamma \int_0^h \big(
% -0.79\norm{v_n(0)}^2_{\Ltwo}
%    +16.33 t^2\norm{\grad f(x_n(0))}_{\Ltwo}^2
%    +0.0001 t\gamma d
%\big)dt + 3\gamma dh \\
%& \leqslant \E\Big[\frac{1}{2}\norm{v_n(0)}^2+f(x_n(0))\Big]
%-0.79 \gamma h\norm{v_n(0)}^2_{\Ltwo}
%+ 5.45 \gamma h^3 \norm{\grad f(x_n(0))}_{\Ltwo}^2
%+ 3.001\gamma dh\\
%& \leqslant \E\Big[\frac{1}{2}\norm{v_n(0)}^2+f(x_n(0))\Big]
%-0.79\gamma h\norm{v_n(0)}^2_{\Ltwo}
%+ 5.45 \gamma h^3 \norm{\grad f(x_n(0))}_{\Ltwo}^2
%+ 3.001 \gamma dh\,.
%\end{align}
%
%Moreover, by \Cref{lem:klmc}, \Cref{lem:6} and Young's inequality, we have
%\begin{align}
%\E[\norm{v_{n+1}(0)}^2-\norm{v_n(h)}^2]
%&=\E[({v_{n+1}(0)}-{v_n(h)})^\top({v_{n+1}(0)}-{v_n(h)}) ]\\
%&\leqslant  \frac{1}{2Lh^2} \norm{v_{n+1}(0)-v_n(h)}^2_{\Ltwo}
%+\frac{Lh^2}{2}\norm{v_n(h)}_{\Ltwo}^2\\
%& \leqslant  \frac{1}{2Lh^2}\Big(0.76 L^2h^4 \norm{v_n(0)}^2_{\Ltwo}
%+ 0.13 L^2h^6 \norm{\grad f(x_n(0))}^2_{\Ltwo}
%+ 0.49 L^2h^5\gamma d\Big) \\
%&\qquad + \frac{Lh^2}{2} \Big(3.07 \norm{v_n(0)}^2_{\Ltwo}
%+ 3.13 h^2\norm{\grad f(x_n(0))}^2_{\Ltwo}
%+ 1.003 h\gamma d\Big)\\
% & \leqslant  1.92 Lh^2 \norm{v_n(0)}^2_{\Ltwo}
%+ 0.001 h^2 \norm{\grad f(x_n(0))}^2_{\Ltwo}
%+ 0.75 Lh^3\gamma d\,.
%\end{align}
%Combining this with \Cref{lem:klmc1} gives
%\begin{align}
%\E\Big[\frac{1}{2}\norm{v_{n+1}(0)}^2+f(x_{n+1}(0))\Big]
% & = \E\Big[\frac{1}{2}\norm{v_n(h)}^2+f(x_n(h))\Big]
%+\frac{1}{2}\E[\norm{v_{n+1}(0)}^2-\norm{v_n(h)}^2]
%+\E[f(x_{n+1}(0))-f(x_n(h))]\\
%& \leqslant  \E\Big[\frac{1}{2}\norm{v_n(0)}^2+f(x_n(0))\Big] \\
%&\qquad -0.79\gamma h \norm{v_n(0)}^2_{\Ltwo}
%+ 5.45 \gamma h^3  \norm{\grad f(x_n(0))}^2_{\Ltwo}
%+ 3.001 \gamma dh \\
%&\qquad + 0.96 Lh^2\norm{v_n(0)}^2_{\Ltwo}
%+ 0.001 h^2 \norm{\grad f(x_n(0))}^2_{\Ltwo}
%+ 0.38 Lh^3\gamma d\\
%&\qquad + 0.58 L^2h^4 \norm{v_n(0)}^2 
%+ 0.183 h^2 \norm{\grad f(x_n(0))}^2_{\Ltwo} + 0.34 L^2h^5\gamma d\\
%& \leqslant  \E\Big[\frac{1}{2}\norm{v_n(0)}^2+f(x_n(0))\Big]
%-0.74 \gamma h \norm{v_n(0)}^2_{\Ltwo}
%+0.43 h^2 \norm{\grad f(x_n(0))}^2_{\Ltwo}
%+ 3.002 h \gamma d\,,
%\end{align}
%where the last step follows from 
%\begin{align}
%Lh^2&\leqslant \gamma^2 h^2\leqslant 0.045 \gamma h \\
%L^3h^6&\leqslant 10^{-6}Lh^2\leqslant 10^{-6}\gamma h\,.
%\end{align}
%This implies
%\begin{align}
%0.74 \gamma h \norm{v_n(0)}^2_{\Ltwo} 
%& \leqslant  \E\Big[\frac{1}{2}\norm{v_n(0)}^2+f(x_n(0))\Big]
%- \E\Big[\frac{1}{2}\norm{v_{n+1}(0)}^2 
%+f(x_{n+1}(0))\Big]
%+0.43 h^2 \norm{\grad f(x_n(0))}^2_{\Ltwo}
%+ 3.002 h \gamma d\,.
%\end{align}
%% Notice that $\E[\norm{v_{k+1}(0)}^2]\leqslant \E[\norm{v_{k}(0)}^2],$
%% $\E[f(x_{k+1}(0))]\leqslant \E[f(x_k(0))],$ and $ e^{-\frac{mh(n-k)}{\gamma}}\le 1$ for $k=0,\dots,n-1,$ we then find
%% \begin{align}
%% e^{-\frac{mh(n-k)}{\gamma}}\norm{v_k(0)}_{\Ltwo}^2
%% & \leqslant 
%% 0.59 \frac{h}{\gamma} e^{-\frac{mh(n-k)}{\gamma}} \norm{\grad f(x_k(0))}^2_{\Ltwo}
%% + 4.06 d e^{-\frac{mh(n-k)}{\gamma}} \\
%% & \qquad +  \frac{1}{0.74\gamma h}\Bigg\{\E\Big[\frac{1}{2}\norm{v_k(0)}^2+f(x_k(0))\Big]
%% - \E\Big[\frac{1}{2}\norm{v_{k+1}(0)}^2 
%% +f(x_{k+1}(0))\Big]\Bigg\}\,.
%% \end{align}
%Summing over $k=0,1,\dots,n-1$ and rearraing the inequality gives
%\begin{align}
%\sum_{k=0}^{n-1}\norm{v_k(0)}_{\Ltwo}^2
%& \leqslant 
%0.59\frac{h}{\gamma} \sum_{k=0}^{n-1} \norm{\grad f(x_k(0))}^2_{\Ltwo} 
%+ 4.06 dn 
%+ \frac{1}{0.74\gamma h}\Bigg\{\E\Big[\frac{1}{2}\norm{v_0(0)}^2+f(x_0(0)) - \frac{1}{2}\norm{v_n(0)}^2-f(x_n(0))\Big] \Bigg\}\,.
%\end{align}
%Note that $v_0(0)=0$ and $f(x_0(0))\leqslant f(x_n(0)),$ it follows that
%\begin{align}
%\sum_{k=0}^{n-1}
%\norm{v_k(0)}_{\Ltwo}^2
%& \leqslant 
%0.59\frac{h}{\gamma} \sum_{k=0}^{n-1}\norm{\grad f(x_k(0))}^2_{\Ltwo} 
%+ 4.06 dn\,.
%\end{align}
%% Also, we note that when $\frac{mh}{\gamma}\leqslant 1,$ it holds that
%% \begin{align}
%% \label{eq:sum_exp1}
%% \sum_{k=0}^{n-1} e^{-\frac{mh(n-k)}{\gamma}}\leqslant \frac{1}{1-e^{-\frac{mh}{\gamma}}}\leqslant \frac{2\gamma}{mh}\,.
%% \end{align}
%% We then arrive at
%% \begin{align}
%% \sum_{k=0}^{n-1}\norm{v_k(0)}_{\Ltwo}^2
%% & \leqslant 
%% 0.59\frac{h}{\gamma} \sum_{k=0}^{n-1} \norm{\grad f(x_k(0))}^2_{\Ltwo} 
%% + 4.06dn  \,.
%% \end{align}
%This completes the proof.
%
%\end{proof}

{\color{blue} This is obsolete.
\begin{proposition}
\label{prop:sum}
Assume the step size $h\leqslant \frac{\gamma}{m}\wedge \frac{1}{4\gamma},$ and $\gamma^2\geqslant 2M.$
It holds that
\begin{align}
\frac{h}{\gamma}\sum_{k=0}^{n-1}
e^{-\frac{mh(n-k)}{\gamma}}
 \norm{ \grad f(\btheta_k)}^2_{\Ltwo}
& \leqslant 
\frac{2.5\gamma}{h}\norm{\btheta_0}^2_{\Ltwo}
+\frac{5\gamma d}{mh}
\\
\sum_{k=0}^{n-1}
e^{-\frac{mh(n-k)}{\gamma}}
\norm{ \bv_k}^2_{\Ltwo}
&\leqslant 
\frac{4.5\gamma}{h}\norm{\btheta_0}^2_{\Ltwo}
+\frac{9.5\gamma d}{mh}\,.
\end{align}
\end{proposition}


\begin{proof}
By Lemma~\ref{lem:sum2}, we have
\begin{align}
    0.6\sum_{k=0}^{n-1}  e^{-mh(n-k)/\gamma}\|\bv_k\|_{\mathbb L_2}^2 
    & \leqslant \frac{2.5d \gamma}{mh} + 
    e^{-\frac{mhn}{\gamma}}\frac{\E[f(\btheta_0)]}{\gamma h}\\
    &\quad + \frac{m}{\gamma^2 }\sum_{k=1}^{n-1} e^{-\frac{mh(n-k)}{\gamma}} \E\Big[2f(\btheta_k) + \|\bv_n\|^2 + 
    \frac{2h(\alpha \gamma - M\beta h)}{\gamma}| \nabla f(\btheta_k)^\top \bv_k|\Big]. 
\end{align}
We first calculate the sum $\frac{m}{\gamma^2}\sum_{k=1}^{n-1} e^{-\frac{mh(n-k)}{\gamma}} \E f(\btheta_k)$ appearing on the right hand side of the previous display.
Note that $f$ is $M$-strongly convex, $\argmin_{\btheta}f(\btheta)=\mathbf{0}$, and $\min_{\btheta}f(\btheta)=0,$ this implies
\begin{align}
f(\btheta)\leqslant \frac{M}{2}\normtwo{\btheta}^2\,.
\end{align}
Notice that
\begin{align}
\normtwo{\btheta_n}^2
\leqslant
\frac{1}{\gamma^2}\Big(\normtwo{\bv_n}^2+
\normtwo{\bv_n+\gamma\btheta_n}^2\Big)\,.
\end{align}
Invoking Lemma~\ref{lem:sum} then yields 
\begin{align}
2\E[f_n]
\leqslant M\norm{\btheta_n}^2_{\Ltwo}
\leqslant
e^{-\frac{mhn}{\gamma}}M\norm{\btheta_0}_{\Ltwo}^2+\frac{dM}{m}\,.
\end{align}
Multiplying both sides of the previous display by $\frac{m}{\gamma^2}e^{-\frac{mh(n-k)}{\gamma}}$ and summing over $k=1,\dots,n-1$ gives
\begin{align}
\frac{2m}{\gamma^2}\sum_{k=1}^{n-1} e^{-\frac{mh(n-k)}{\gamma}} \E f_n
\leqslant
\frac{nmM}{\gamma^2}e^{-\frac{mhn}{\gamma}}\norm{\btheta_0}^2_{\Ltwo}+\frac{dM}{\gamma^2}\sum_{k=1}^{n-1}e^{-\frac{mh(n-k)}{\gamma}}\,.
\end{align}
When $\frac{mh}{\gamma}<1$ and $\gamma^2\geqslant 2M,$ it follows that
\begin{align}
\frac{2m}{\gamma^2}\sum_{k=1}^{n-1} e^{-\frac{mh(n-k)}{\gamma}} \E f_n
&\leqslant
\frac{M}{2\gamma h}\norm{\btheta_0}^2_{\Ltwo}+\frac{\gamma d}{mh}
\leqslant \frac{\gamma}{4h}
\norm{\btheta_0}^2_{\Ltwo}
+\frac{\gamma d}{mh}\,.
\end{align}
Similarly, one can derive that
\begin{align}
\frac{m}{\gamma^2}\sum_{k=1}^{n-1} e^{-\frac{mh(n-k)}{\gamma}} \norm{\bv_k}_{\Ltwo}^2
\leqslant
\frac{2\gamma}{h}\norm{\btheta_0}^2_{\Ltwo}
+\frac{2\gamma d}{mh}\,.
\end{align}
 Note that
 \begin{align}
 \frac{2h(\alpha \gamma - M\beta h)}{\gamma}| \nabla f(\btheta_k)^\top \bv_k|
 \leqslant 2h| \nabla f(\btheta_k)^\top \bv_k|
 \leqslant 
\frac{(2h\alpha)^2\normtwo{\grad f(\btheta_k)}^2}{2}
 + \frac{\normtwo{\bv_k}^2}{2}\,,
 \end{align}
 and 
 \begin{align}
\normtwo{\grad f(\btheta_k)}^2
\leqslant
M^2\normtwo{\btheta_k}^2\,.
  \end{align}
Using the same trick, one can verify that
\begin{align}
\frac{m}{\gamma^2}\sum_{k=1}^{n-1} e^{-\frac{mh(n-k)}{\gamma}}  \frac{2h(\alpha \gamma - M\beta h)}{\gamma}| \nabla f(\btheta_k)^\top \bv_k|
 \leqslant 
 \frac{2\gamma}{h}\norm{\btheta_0}^2_{\Ltwo}
 + \frac{2\gamma d}{mh}\,.
\end{align}
Collecting pieces then gives
\begin{align}
 0.6\sum_{k=0}^{n-1}  e^{-\frac{mh(n-k)}{\gamma}}\|\bv_k\|_{\mathbb L_2}^2 
 \leqslant
\frac{2.5\gamma}{h}\norm{\btheta_0}^2_{\Ltwo}
+\frac{5.5\gamma d}{mh}\,.
\end{align}
By Lemma~\ref{lem:sum2}, we  also obtain that
\begin{align}
1.1 \frac{h}{\gamma} 
    \sum_{k=0}^{n-1} e^{-\frac{mh(n-k)}{\gamma}} \|\nabla f(\btheta_k)\|_{\mathbb L_2}^2
\leqslant 
\frac{2.5\gamma}{h}\norm{\btheta_0}^2_{\Ltwo}
+\frac{5.5\gamma d}{mh}\,.
\end{align}
This completes the proof.
\end{proof}
}

\begin{theorem}
\label{thm:klmc1}
\textbf{[Checked by Arnak on April 15th]}
Assume $f$ is $m$-strongly convex and $M$-smooth.
Set $\gamma^2 \geqslant 2M$ and  $h\leqslant \frac{1}{4\gamma}$.  It holds that
\begin{align}
    W_2(\nu_n^{\textup{KLMC}},\pi) &\leqslant 
    \sqrt{2}\varrho^n  W_2(\nu_0,\pi)  + 
    \frac{5Mh \sqrt{2 p}}{m} + \frac{5
    M h \rho^{n/2}}{\sqrt{m}} \bigg\{ 
    \|\btheta_0-\btheta^*\|_{\mathbb L_2}^2 +  
    \gamma^{-2}\|\bv_0\|_{\mathbb L_2}^2  \bigg\}^{1/2}
\end{align}
where $\nu_n^{\textup{KLMC}}$ denotes the distribution of $\btheta_k$ and  $\varrho = \exp(-mh/\gamma)$.
\end{theorem}

\red{ADD REMARK: EITHER DECOMPOSE $W_2(\nu_0,\pi)$ or $\norm{\btheta_0-\btheta^*}_{\Ltwo}^2$ }



\begin{corollary}
Assume the assumptions stated in Theorem~\ref{thm:klmc1} hold, $\nu_0$ is the Dirac mass at the minimum point of $f$, and set $m=1.$ 
Given a small target precision level $\epsilon\in(0,1),$
 for any step size
\begin{align}
h=\frac{ \epsilon}{85M}\,,
\end{align}
it holds that
\begin{align}
 W_2(\nu_n,\pi)\le \sqrt{d}\epsilon\,,
\end{align}
 provided that the number of iterations
\begin{align}
n \geqslant \frac{2\gamma}{h}\log \Big(\frac{2}{\epsilon}\Big)\,.
\end{align}
\end{corollary}
\begin{proof}[Proof of~\Cref{thm:klmc1}]
Let $\btheta_n,\bv_n$ be the iterates of KLMC algorithm.
Let $(\bar\btheta_n,\bar\bv_n)$ be the $n$-th step of the exact underdamped Langevin diffusion, coupled with $(\btheta_n,\bv_n)$ through the same Brownian motion and starting from a random point $(\bar\btheta_0,\bar\bv_0)\propto \exp(-f(\by)+\frac{1}{2}\norm{\bw}^2)$ such that $\bar\bv_0=\bv_0$. 
Let $(\btheta_{n+1}^*,\bv_{n+1}^*)$ be the 1-step exact Langevin diffusion starting from $(\btheta_n,\bv_n).$

Define $A_n>0$ by  $A_n^2 = \|\bv_n-\bar\bv_n 
+ \gamma (\btheta_{n}-\bar\btheta_n) \|_{\mathbb L_2}^2 + 
\norm{ \bv_n-\bar\bv_{n}}_{\mathbb L_2}^2$ and $\varrho = \exp(-mh/\gamma)$. The triangle inequality 
yields
\begin{align}
    A_n &\leqslant \big(\norm{\bv_n^*-\bar\bv_n 
+ \gamma(\btheta_{n}^*- \bar\btheta_n)}_{\mathbb L_2}^2 + 
\norm{ \bv_n-\bar\bv_{n}}_{\mathbb L_2}^2 \big)^{1/2} + \big(\norm{\bv_n-\bv_n^* 
+ \gamma (\btheta_{n}- \btheta_n^*)}_{\mathbb L_2}^2 + 
\norm{ \bv_n - \bv_{n}^*}_{\mathbb L_2}^2 \big)^{1/2} \\
&\leqslant \varrho A_{n-1}  + 
\big(\norm{\bv_n-\bv_n^* 
+ \gamma (\btheta_{n}- \btheta_n^*)}_{\mathbb L_2}^2 + 
\norm{ \bv_n - \bv_{n}^*}_{\mathbb L_2}^2 \big)^{1/2}\\
&\leqslant \varrho A_{n-1}  + 
\sqrt{2}
\norm{ \bv_n - \bv_{n}^*}_{\mathbb L_2}^2  + \gamma\norm{ \btheta_{n}- \btheta_n^*}_{\mathbb L_2},
\end{align}
where the second inequality follows from the
proof of Proposition 1 in~\cite{dalalyan_riou_2018}, while the third inequality is a consequence of the 
triangle inequality and the following elementary inequality $\sqrt{(a+b)^2 + c^2}\leqslant \sqrt{a^2 + c^2} + b$ for 
$a,b,c\geqslant 0$. From the last display, we infer that
\begin{align}\label{eq:klmc_ctr}
    A_n 
&\leqslant \varrho^n A_{0}  + 
\sum_{k=1}^n \varrho^{n-k}\big(\sqrt{2}
\norm{ \bv_k - \bv_{k}^*}_{\mathbb L_2} 
+ \gamma\norm{ \btheta_{k}- \btheta_k^*}_{\mathbb L_2}\big),
\end{align}
By \Cref{lem:klmc} and $Mh^2\leqslant (\gamma h)^2/2 \leqslant 1/32$,
\begin{align}
\norm{\bv_{k+1}-\bv_{k+1}^*}_{\Ltwo}
& \leqslant  Mh^2 (1.02\sqrt{p}
+ 0.51 \norm{\bv_k}_{\Ltwo}
+0.21 h\norm{\grad f(\btheta_k)}_{\Ltwo}) \\
\norm{\btheta_{k+1}-\btheta_{k+1}^*}_{\Ltwo}
& \leqslant  Mh^3 (0.06\sqrt{p}
+ 0.17\norm{\bv_k}_{\Ltwo}
+0.043 h\norm{\grad f(\btheta_k)}_{\Ltwo}) \,.
\end{align}
Therefore,
\begin{align}
    \sqrt{2}
\norm{ \bv_k - \bv_{k}^*}_{\mathbb L_2} 
+ \gamma\norm{ \btheta_{k}- \btheta_k^*}_{\mathbb L_2} &\leqslant 
Mh^2 \big((1.02\sqrt{2} + 0.06\cdot 0.25 )\sqrt{p}
+ (0.51\sqrt{2} + 0.17\cdot 0.25) \norm{\bv_k}_{\Ltwo}\\
&\qquad + (0.21\sqrt{2} + 0.043\cdot 0.25) h\norm{\grad f(\btheta_k)}_{\Ltwo}) \\
&\leqslant 
0.73 Mh^2 \big(2\sqrt{p}
+  \norm{\bv_k}_{\Ltwo} + 0.43h\norm{\grad f(\btheta_k)}_{\Ltwo}).
\end{align}
This inequality, in conjunction with 
\eqref{eq:klmc_ctr}, implies that
\begin{align}\label{eq:klmc_ctr1}
    A_n 
&\leqslant \gamma \varrho^n  W(\nu_0,\pi)  + 
0.73 Mh^2\sum_{k=1}^n \varrho^{n-k}\big(2\sqrt{p} + 
\norm{ \bv_k}_{\mathbb L_2} 
+ 0.43 h\norm{ \nabla f(\btheta_{k})}_{\mathbb L_2}\big)\\
&\leqslant \varrho^n \gamma W(\nu_0,\pi)  + 
\frac{1.46 Mh^2\sqrt{p}}{1-\varrho} + 0.73 Mh^2\sum_{k=1}^n \varrho^{n-k}\big(\norm{ \bv_k}_{\mathbb L_2} 
+ 0.43 h\norm{ \nabla f(\btheta_{k})}_{\mathbb L_2}\big)\\
&\leqslant \varrho^n \gamma W(\nu_0,\pi)  + 
\frac{1.46 Mh^2\sqrt{p}}{1-\varrho} + 0.75 Mh^2\sum_{k=1}^n \varrho^{n-k}\big(\norm{ \bv_k}_{\mathbb L_2}^2 
+ 7 h^2\norm{ \nabla f(\btheta_{k})}_{\mathbb L_2}^2\big)^{1/2}\\
&\leqslant \varrho^n \gamma W(\nu_0,\pi)  + 
\frac{1.46 Mh^2\sqrt{p}}{1-\varrho} + \frac{0.75 Mh^2}{\sqrt{1-\varrho}}
\bigg\{\sum_{k=1}^n \varrho^{n-k}\big(\norm{ \bv_k}_{\mathbb L_2}^2 
+ 7 h^2\norm{ \nabla f(\btheta_{k})}_{\mathbb L_2}^2\big)\bigg\}^{1/2}.
\end{align}
Since $m\leqslant M \leqslant \gamma^2/2$ 
and $\gamma h\leqslant 1/4$, we have 
$mh/\gamma \leqslant Mh/\gamma \leqslant (\gamma h)/2\leqslant 1/8$. Therefore, 
$\varrho \leqslant 1 - 0.94 mh/\gamma $ and 
\begin{align}\label{eq:klmc_ctr2}
    A_n 
&\leqslant \varrho^n \gamma W(\nu_0,\pi)  + 
\frac{1.56 Mh\gamma \sqrt{p}}{m} + 0.78 M h^2
\bigg\{\frac{\gamma}{mh} \sum_{k=1}^n \varrho^{n-k}\big(\norm{ \bv_k}_{\mathbb L_2}^2 
+ 7 h^2\norm{ \nabla f(\btheta_{k})}_{\mathbb L_2}^2\big)\bigg\}^{1/2}.
\end{align}
We can apply \Cref{lem:sum2} to infer that
\begin{align}\label{eq:klmc_ctr2}
    A_n &\leqslant \varrho^n \gamma W(\nu_0,\pi)  
    + \frac{1.56 Mh\gamma \sqrt{p}}{m} + \frac{3.35 
    M\gamma h}{\sqrt{m}} \bigg\{\frac{ p}{m} + 
    \rho^n \big(\|\btheta_0-\btheta^*\|_{\mathbb 
    L_2}^2 +  \gamma^{-2}\|\bv_0\|_{\mathbb L_2}^2 
    \big) \bigg\}^{1/2}\\
    &\leqslant \varrho^n \gamma W(\nu_0,\pi)  + 
    \frac{5Mh\gamma \sqrt{p}}{m} + \frac{3.35 
    M\gamma h \rho^{n/2}}{\sqrt{m}} \bigg\{ 
    \|\btheta_0-\btheta^*\|_{\mathbb L_2}^2 +  
    \gamma^{-2}\|\bv_0\|_{\mathbb L_2}^2  \bigg\}^{1/2}
\end{align}
Finally, one can check that $2A_n^2\geqslant \gamma^2 
\|\btheta_n - \bar\btheta_n\|_{\mathbb L_2}^2 \geqslant 
\gamma^2 W_2^2(\nu_n^{\textup{KLMC}},\pi)$. This 
completes the proof of the theorem. 
\end{proof}





\clearpage


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End:

==> code.tex <==
N_LMC = 1
N_RLMC = 1
eps = 0.1
for (i in 1:6)
{
  kappa = 10^(2*i-1)
  N_RLMC = (3*kappa/eps)+(3.8*kappa^(4/3)/eps^(2/3))
  N_RLMC = N_RLMC*log(20/eps)
  N_RLMC = round(N_RLMC)
  
  N_LMC = (2.2*kappa/eps^2)
  N_LMC = N_LMC*log(20/eps)
  N_LMC = round(N_LMC)
  
  gamma_x_h = eps/(sqrt(kappa))
  N_KLMC = 5*kappa*log(20/eps)
  N_KLMC = N_KLMC /(gamma_x_h)
  N_KLMC = round(N_KLMC)
  cat('****','\n')
  
  sqt_kap = sqrt(kappa)
  gamma_x_h = sqrt(4.6*eps*sqt_kap + 625)
  gamma_x_h = (gamma_x_h - 25)/sqt_kap
  gamma_x_h = gamma_x_h^(2/3)
  N_RKLMC = 10*kappa*log(1/(c*eps))
  N_RKLMC = N_RKLMC /(gamma_x_h)
  N_RKLMC = round(N_RKLMC)
  cat('****','\n')
  cat('N_LMC  = ', N_LMC,'\n')
  cat('N_RLMC = ', N_RLMC,'\n')
  cat('N_KLMC = ', N_KLMC,'\n')
  cat('N_RKLMC = ', N_RKLMC,'\n')
}
**************************************************
*************** eps = 0.1 ************************
**************************************************
**** 
**** 
N_LMC  =  11656 
N_RLMC =  3603 
N_KLMC =  8377 
N_RKLMC =  10493 
**** 
**** 
N_LMC  =  1165630 
N_RLMC =  1093469 
N_KLMC =  8377375 
N_RKLMC =  1052908 
**** 
**** 
N_LMC  =  116562982 
N_RLMC =  449660344 
N_KLMC =  8377375322 
N_RKLMC =  108708094 
**** 
**** 
N_LMC  =  11656298206 
N_RLMC =  202925555139 
N_KLMC =  8.377375e+12 
N_RKLMC =  13201497605 
**** 
**** 
N_LMC  =  1.16563e+12 
N_RLMC =  9.361087e+13 
N_KLMC =  8.377375e+15 
N_RKLMC =  2.163975e+12 
**** 
**** 
N_LMC  =  1.16563e+14 
N_RLMC =  4.339243e+16 
N_KLMC =  8.377375e+18 
N_RKLMC =  4.245782e+14

**************************************************
*************** eps = 0.001 **********************
**************************************************

N_LMC  =  217876726 
N_RLMC =  378183 
N_KLMC =  1565879 
N_RKLMC =  451945 
**** 
**** 
N_LMC  =  21787672616 
N_RLMC =  67343715 
N_KLMC =  1565878872 
N_RKLMC =  45196067 
**** 
**** 
N_LMC  =  2.178767e+12 
N_RLMC =  20438854816 
N_KLMC =  1.565879e+12 
N_RKLMC =  4521183289 
**** 
**** 
N_LMC  =  2.178767e+14 
N_RLMC =  8.404943e+12 
N_KLMC =  1.565879e+15 
N_RKLMC =  453684491181 
**** 
**** 
N_LMC  =  2.178767e+16 
N_RLMC =  3.793036e+15 
N_KLMC =  1.565879e+18 
N_RKLMC =  4.68409e+13 
**** 
**** 
N_LMC  =  2.178767e+18 
N_RLMC =  1.749752e+18 
N_KLMC =  1.565879e+21 
N_RKLMC =  5.688353e+1 

**************************************************
*************** eps = 0.00001 ********************
**************************************************
**** 
**** 
N_LMC  =  3.191905e+12 
N_RLMC =  46085016 
N_KLMC =  229402021 
N_RKLMC =  14605230 
**** 
**** 
N_LMC  =  3.191905e+14 
N_RLMC =  5540399632 
N_KLMC =  2.29402e+11 
N_RKLMC =  1460523523 
**** 
**** 
N_LMC  =  3.191905e+16 
N_RLMC =  986588726220 
N_KLMC =  2.29402e+14 
N_RKLMC =  146052862163 
**** 
**** 
N_LMC  =  3.191905e+18 
N_RLMC =  2.994302e+14 
N_KLMC =  2.29402e+17 
N_RKLMC =  1.46058e+13 
**** 
**** 
N_LMC  =  3.191905e+20 
N_RLMC =  1.231328e+17 
N_KLMC =  2.29402e+20 
N_RKLMC =  1.461089e+15 
**** 
**** 
N_LMC  =  3.191905e+22 
N_RLMC =  5.556816e+19 
N_KLMC =  2.29402e+23 
N_RKLMC =  1.46615e+17
